The Curse of Correlations for Robust Fingerprinting of Relational Databases

Database fingerprinting have been widely adopted to prevent unauthorized sharing of data and identify the source of data leakages. Although existing schemes are robust against common attacks, like random bit flipping and subset attack, their robustness degrades significantly if attackers utilize the inherent correlations among database entries. In this paper, we first demonstrate the vulnerability of existing database fingerprinting schemes by identifying different correlation attacks: column-wise correlation attack, row-wise correlation attack, and the integration of them. To provide robust fingerprinting against the identified correlation attacks, we then develop mitigation techniques, which can work as post-processing steps for any off-the-shelf database fingerprinting schemes. The proposed mitigation techniques also preserve the utility of the fingerprinted database considering different utility metrics. We empirically investigate the impact of the identified correlation attacks and the performance of mitigation techniques using real-world relational databases. Our results show (i) high success rates of the identified correlation attacks against existing fingerprinting schemes (e.g., the integrated correlation attack can distort 64.8\% fingerprint bits by just modifying 14.2\% entries in a fingerprinted database), and (ii) high robustness of the proposed mitigation techniques (e.g., with the mitigation techniques, the integrated correlation attack can only distort $3\%$ fingerprint bits).

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle


==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}


In this paper, we have proposed robust fingerprinting for relational databases. First, we have validated  the vulnerability of existing database fingerprinting schemes by identifying different correlation attacks: column-wise correlation attack (which utilizes the joint distributions among attributes), row-wise correlation attack (which utilizes the statistical relationships among the rows), and integration of them. Next, to defend against the identified attacks, we have  developed mitigation techniques that can work as post-processing steps for any off-the-shelf database fingerprinting schemes. Specifically, the column-wise mitigation technique modifies limited entries in the fingerprinted database by solving a set of optimal mass transportation problems concerning pairs of marginal distributions. On the other hand, the row-wise  mitigation technique modifies a small fraction of the fingerprinted database entries by solving a combinatorial search problem. We have also empirically investigated the impact of the identified correlation attacks and the performance of proposed mitigation techniques on an real-world relational database. Experimental results show high success rates for the correlation attacks and high robustness for the proposed mitigation techniques, which alleviate the  attacks   having access to correlation models directly calculated from the data.



% even using inaccurate/noisy data correlations.  
 
 
 
\begin{acks}
Research reported in this publication was supported by the National Library Of Medicine of the National Institutes of Health under Award Number R01LM013429.
\end{acks}

==> sections/evaluation.tex <==



\section{Evaluation}
\label{sec:eva}
Now, we evaluate the   correlation attacks and the   robust fingerprinting mechanisms, investigate their impact on fingerprint robustness and  database utility, and empirically study  the effect of   knowledge asymmetry between the  database owner and a malicious SP.


 
\subsection{Experiment Setup}
 


We consider   a Census database \cite{asuncion2007uci} as the study case. 
As discussed in Section \ref{sec:vanilla}, we choose the state-of-the-art scheme developed in \cite{li2005fingerprinting} as the vanilla mechanism, because it is shown to be robust against common attacks (such as random bit flipping, subset, and superset attacks).
% and it adopts majority voting on the fingerprinted entries to detect the fingerprint  bit-string.  
We use 128-bits fingerprint   string  ($L=128$) for    the vanilla   scheme, because when considering $N$ SPs, as long as $L> \ln N$, the vanilla scheme can thwart exhaustive search and various types of attacks \cite{li2005fingerprinting}, and in most cases a 64-bits fingerprint string is shown to provide high robustness. 
% \hlgreen{In all the experiments, we let all attacks, i.e.,  $\mathrm{Atk_{rnd}}$, $\mathrm{Atk_{col}}(\mathcal{J})$, and $\mathrm{Atk_{row}}(\mathcal{S})$  change only the LSB of database entries, since the fingerprint bits are added in the LSB of the selected entries by the vanilla scheme (as discussed in Section \ref{sec:vanilla}). Please refer to Appendix \ref{sec:utility_LSB} for the validation that fingerprinting LSBs achieves the highest  utility for the Census database.}

% We also let $\mathrm{Dfs_{col}}(\mathcal{J}')$ change only the LSB of database entries, because it   usually change large amount of database entries (about ). Whereas, $\mathrm{Atk_{row}}(\mathcal{S})$ and $\mathrm{Dfs_{row}}(\mathcal{S}')$ can change a database entry to all its possible values, because such techniques change limited number of entries (and hence they do not significantly degrade database utility).




In different experiments, to distinguish different instances of the row-wise and column-wise correlations, we also parametrize $\mathcal{J}'$, $\mathcal{S}'$, $\mathcal{J}$, and $\mathcal{S}$  when specifying their resources. For instance,    $\mathcal{J}'(\mathbf{R})$   indicates Alice's prior knowledge on column-wise correlations   are  calculated directly from the original database.




% the vanilla fingerprint scheme (also describe in background) \hl{EA: also say, why you selected this particular one and not another one}

% \hl{The main evaluation should be for the complete attack (including both row-wise and column-wise correlations). Under that, we can also separately show the results of only row or column-wise correlation attack.}


 
\subsection{Evaluations on Census Database}
\label{sec:census_study}

%\hl{EA: I didnt read after this yet}

Census database \cite{asuncion2007uci}  records 14 discrete or categorical attributes of 32561 individuals.  To add fingerprint to this database, Alice first encodes the values of each attribute as integers in a way that the LSB carries the least information. {\color{black}Recall that to achieve high database utility, we let the vanilla scheme only fingerprint the LSBs (in Appendix \ref{sec:utility_LSB} we validate that fingerprinting the other bits reduces database utility).} In particular, for a discrete numerical attribute (e.g., age), the values are first sorted in an ascending order and then divided into   non-overlapping ranges, which are then encoded as ascending  integers starting from 0. For a categorical attribute (e.g., marital-status),  the instances are first mapped to a high dimensional space via the word embedding technique \cite{mikolov2013distributed}. Words having similar meanings appear roughly in the same area of the   space. After mapping, these vectors are clustered into a hierarchical tree structure, where each leaf node represents an instance of that attribute and is encoded by an integer and the adjacent leaf nodes differ in the LSB.    Besides, we use K-means   to group the individuals in the Census database into non-overlapping communities, and according to the Schwarz's Bayesian inference criterion (BIC) \cite{schwarz1978estimating}, the optimal number of communities is $C=10$.  


\begin{table*}[htb]
% \resizebox{\columnwidth}{!}{
\begin{center}
 \begin{tabular}{c|c | c|c| c | c | c| c| c| c| c  } 
 \hline
 \hline
 Attack on           &   robustness  \&  & using &  \multicolumn{8}{c}{    rounds of $\mathrm{Atk_{col}}\Big(    \mathcal{J}(\mathbf{R}) \Big)$} \\
\cline{4-11}
 $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$ &   utility loss & $\mathrm{Atk_{row}}\Big(   \mathcal{S}(\mathbf{R}) \Big)$  & 1&2&3&4&5&6&7&8 \\
 \hline
using & $\mathrm{num_{cmp}}$ & \multirow{3}{*}{N/A }  &  28  &  43 &   55   & 58   & 63   & 74 &   77  & \cellcolor{Green}82  \\ 
\multirow{2}{*}{$\mathrm{Atk_{col}}\Big(\mathcal{J}(\mathbf{R})\Big)$} & $r$  &    & u     &      u     &      u    & <  0.08\%    &  <  0.73\%   & <  53.2\%   & < 71.8\%   & < \cellcolor{Green}91.4\%   \\
  & $\mathrm{per_{chg}}$ & & \cellcolor{Gray}$4.4\%$ & \cellcolor{Gray}$10.9\%$ & \cellcolor{Gray}$14.2\%$ &  \cellcolor{Gray}$15.9\%$ &  \cellcolor{Gray}$18.4\%$ & \cellcolor{Gray}$23.7\% $ & \cellcolor{Gray}$25.3\%$ & \cellcolor{Gray}$27.1\%$\\
  \hline
using $\mathrm{Atk_{row}}\Big(   \mathcal{S}(\mathbf{R}) \Big)$ & $\mathrm{num_{cmp}}$ &     \cellcolor{Blue}78   &   78  &  79   & 80    &81   & 82  &  83  &  83  &  \cellcolor{Red}83 \\ 
  \multirow{2}{*}{ and  $\mathrm{Atk_{col}}\Big(\mathcal{J}(\mathbf{R})\Big)$} &  $r$    & \cellcolor{Blue}< $82.9\%$  &  < 82.9\%   & <  89.1\%  & < 89.4\%  & < 90.1\%    &<  91.4\%  & < 93.7\%  & < 93.7\%  & \cellcolor{Red}< 93.7\%   \\
 & $\mathrm{per_{chg}}$ & \cellcolor{Blue}2.9\% & 8.9\% & 10.5\%  & 11.3\% & 11.5\% & 11.9\% & 12.6\% & 13.7\% & \cellcolor{Red}14.2\%\\
  \hline
  \hline
\end{tabular}
\end{center}
% }
\caption{Fingerprint robustness and utility loss of different correlation attacks on the vanilla fingerprinted Census database $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$. The fingerprint robustness  metrics are the  number of compromised fingerprint bits, i.e.,  $\mathrm{num_{cmp}}$ and i.e., accusable ranking $r$. The   utility loss of the malicious SP is the  fraction of modified entries as a result of the attack, i.e., $\mathrm{per_{chg}} = 1-Acc(\overline{\mathbf{R}})$. `u' stands for uniquely accusable. `< $r$' means top $r$ accusable.} 
\label{table:correlation_attack_compare}
\end{table*}

 
\subsubsection{Impact of Correlation Attacks on Census Database}
\label{sec: int_attack_census}

% We first compare  the performance of the integrated correlation attack  with $\mathrm{Atk_{row}}(\mathcal{S})$ and $\mathrm{Atk_{col}}(\mathcal{J})$. Then, we  investigate the impact  of $\mathrm{Atk_{row}}(\mathcal{S})$ and $\mathrm{Atk_{col}}(\mathcal{J})$ separately. 

We first study  the impact  of $\mathrm{Atk_{row}}(\mathcal{S})$ and $\mathrm{Atk_{col}}(\mathcal{J})$, and then present the impact of the integration of them.  In this experiment, we assume that the malicious SP  has the ground truth knowledge about the row- and column-wise correlations, i.e., it has access to $\mathcal{S}$ and $\mathcal{J}$ that  are directly computed from $\mathbf{R}$. 
As a result, we represent its prior knowledge as  $\mathcal{S}(\mathbf{R})$ and $\mathcal{J}(\mathbf{R})$. By launching  the  row-wise,  column-wise, and integrated correlation attack, the  malicious SP   generates  pirated database      $\overline{\mathbf{R}}\Big(\mathrm{FP},\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R})),\emptyset)\Big)$,   $\overline{\mathbf{R}}\Big(\mathrm{FP},\emptyset,\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))\Big)$, and $\overline{\mathbf{R}}\Big(\mathrm{FP},\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R})),\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))\Big)$, respectively. 
%We will study the case where the malicious SP has inaccurate prior knowledge in Section \ref{sec:knowledge_asym}.

%(which combines $\mathrm{Atk_{row}}(\mathcal{S},C)$ and $\mathrm{Atk_{col}}(\mathbb{J})$)

% \hl{EA: in all following experiments, you are only changing LSB. Lets add it somewhere.}  



\noindent\textbf{Impact of $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$.} 
%{on fingerprint robustness and database utility.}
% In this experiment example, we consider the malicious SP's prior knowledge on the column-wise correlation is calculated from a noisy (random) database, i.e., $\mathbf{R}_\kappa$, which is obtained from $\mathbf{R}$ by randomly removing $\kappa$ fraction of the data records. For example, by randomly removing $5\%$ of records from $\mathbf{R}$, we have an instance of 
% $\mathbf{R}_{0.05}$. Clearly, $\mathbf{R}_{0} = \mathbf{R}$. Thus, we represent the malicious SP's  column-wise prior knowledge as $\mathcal{J}(\mathbf{R}_\kappa)$.
First, we validate that $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$ is more powerful than the   random bit flipping attack $\mathrm{Atk_{rnd}}$ discussed in Section \ref{sec:system-threat}. 
% which randomly changes entries of fingerprinted database to other values of the attributes. 
{\color{black}We set the threshold $\tau_{\mathrm{col}}^{\mathrm{Atk}} = 0.0001$ when comparing  $|J_{p,q}(a,b)-\widetilde{J_{p,q}}(a,b)|$.\footnote{{\color{black}In all experiments, we choose a small value for $\tau_{\mathrm{col}}^{\mathrm{Atk}}$, $\tau_{\mathrm{col}}^{\mathrm{Dfs}}$, and $\tau_{\mathrm{col}}$, because a database usually contains     thousands of data records and the addition of fingerprint changes a small fraction of entries, which does not cause large changes in the joint distributions. On the contrary, we choose a large value for $\tau_{\mathrm{row}}^{\mathrm{Atk}}$  and $\tau_{\mathrm{row}}$, because the statistical relationship is defined as an exponentially decay function, which ranges from 0 to 1, and the added fingerprint results in a larger change for this  statistical relationship.}} As a result, it takes 8 iterations (attack rounds) for $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$ to converge (i.e., stop including new suspicious fingerprinted positions in $\mathcal{P}$).} In Table \ref{table:correlation_attack_compare}, we record the fingerprint robustness  (i.e.,  $\mathrm{num_{cmp}}$ and   $r$) and utility loss of the malicious SP (fraction of modified entries as a result of the attack, i.e.,  $\mathrm{per_{chg}} = 1-Acc(\overline{\mathbf{R}})$) when launching increasing rounds of $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$ 
 on the vanilla fingerprinted Census database. We observe that with more attack rounds, more fingerprint bits are compromised, and the accusable ranking of the malicious SP also decreases, which suggests that Alice may accuse innocent SP with increasing probability.   In Table \ref{table:atk_rnd}, we present the performance of $\mathrm{Atk_{rnd}}$ on the vanilla  fingerprinted   database. Specifically, by setting the fraction of entries changed ($\mathrm{per_{chg}}$) due to $\mathrm{Atk_{rnd}}$  equal to that of $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$ with increasing rounds (i.e., the cells highlighted in gray in Table \ref{table:correlation_attack_compare}), we calculated $\mathrm{num_{cmp}}$ and $r$ achieved by $\mathrm{Atk_{rnd}}$. 

\begin{table}[htb]
\begin{center}
 \begin{tabular}{c | c|c| c | c | c| c } 
 \hline
 \hline
 $\mathrm{per_{chg}}$&    $\leq14.2\%$ &  $15.9\%$ &  $18.4\%$ & $23.7\% $ & $25.3\%$ &  $27.1\%$ \\
 \hline
 $\mathrm{num_{cmp}}$ &  0    &1   & 1  &  2  &  3  &   4 \\ 
$r$ &    u   & u    & u  &u   & u  & u    \\
  \hline
  \hline
\end{tabular}
\caption{Performance and cost of  $\mathrm{Atk_{rnd}}$ on the vanilla fingerprinted Census database. $\mathrm{per_{chg}}$ values are set to be equal to that of  $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$  (cells highlighted in gray in Table \ref{table:correlation_attack_compare}). $r=\text{u}$ means uniquely accusable.} 
\label{table:atk_rnd}
\end{center}
\end{table}

Combining  Tables \ref{table:correlation_attack_compare}  and \ref{table:atk_rnd}, we observe that if $\mathrm{per_{chg}}$ is below $14.2\%$, $\mathrm{Atk_{rnd}}$ cannot compromise any fingerprint bits, whereas $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$ compromises 28 fingerprint bits (out of 128).  Even when $\mathrm{per_{chg}} = 27.1\%$, $\mathrm{Atk_{rnd}}$ can only distort 4 fingerprint bits. As a result, if the malicious SP launches $\mathrm{Atk_{rnd}}$, it will be uniquely accusable for pirating the database. 
Whereas, when $\mathrm{per_{chg}} = 27.1\%$  $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$ distorts 82 bits, which makes the malicious SP only rank top $91.4\%$ accusable and will cause Alice accuse innocent SP with very high probability (the cells highlighted in green in Table \ref{table:correlation_attack_compare}).  
In fact, for $\mathrm{Atk_{rnd}}$ to compromise enough fingerprint bits so as to cause Alice to accuse innocent SPs, it needs to flip more than $83\%$ of the entries in the fingerprinted Census database. Clearly, the vanilla fingerprint scheme is robust against $\mathrm{Atk_{rnd}}$, however, its robustness significantly degrades against $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$.

\begin{figure}
  \begin{center}
  \begin{tabular}{ccc}
     \includegraphics[width= .31\columnwidth,height=2.5cm]{figures/P_col_atkcol_vs_atkrnd-eps-converted-to.pdf}
		&
		     \includegraphics[width= .31\columnwidth,height=2.5cm]{figures/P_row_atkcol_vs_atkrnd-eps-converted-to.pdf}
		&
     \includegraphics[width= .31\columnwidth,height=2.5cm]{figures/P_cov_atkcol_vs_atkrnd-eps-converted-to.pdf}
     \\
    {\small  (a) $\mathrm{P_{col}}$ }  &
    {\small  (b) $\mathrm{P_{row}}$ } &
    {\small  (c) $\mathrm{P_{cov}}$ }\\
    % {column correlations.} &
    %  {row correlations.} &
    %   {covariance matrix.}\\
        \end{tabular}
      \end{center}
  \caption{\label{fig:atkcol_vs_atkrnd}  Comparison of (a) $\mathrm{P_{col}}$, (b) $\mathrm{P_{row}}$, and (c) $\mathrm{P_{cov}}$ achieved by $\overline{\mathbf{R}}(\emptyset,\emptyset,\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R})))$ and  $\overline{\mathbf{R}}(\mathrm{Atk_{rnd}},\emptyset,\emptyset)$ when $\mathrm{per_{chg}}$ are set as the values highlighted in gray in Table \ref{table:correlation_attack_compare}.}
\end{figure}


In Figure \ref{fig:atkcol_vs_atkrnd}, by setting  $\mathrm{per_{chg}}$ to the values highlighted in gray in Table \ref{table:correlation_attack_compare}, 
we compute and compare  the    {\color{black}utility of the pirated database (i.e, $\mathrm{P_{col}}(\overline{\mathbf{R}})$ for $\tau_{\mathrm{col}} = 0.0001$, $\mathrm{P_{row}}(\overline{\mathbf{R}})$ for $\tau_{\mathrm{row}} = 10$,  and $\mathrm{P_{cov}}(\overline{\mathbf{R}})$)} obtained from the  vanilla fingerprinted database after $\mathrm{Atk_{rnd}}$ and $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$, i.e., $\overline{\mathbf{R}}(\mathrm{Atk_{rnd}},\emptyset,\emptyset)$ and $\overline{\mathbf{R}}(\emptyset,\emptyset,\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R})))$. We also plot the utility of the vanilla fingerprinted database %(after fingerprinting) 
using black lines as the benchmark ($\mathrm{P_{col}}(\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset))=0.95$, $\mathrm{P_{row}}(\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset))=1.00$, and $\mathrm{P_{cov}}(\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset))=0.99$). Clearly, $\overline{\mathbf{R}}(\emptyset,\emptyset,\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R})))$ always achieves higher utility values than $\overline{\mathbf{R}}(\mathrm{Atk_{rnd}},\emptyset,\emptyset)$, and it has similar utility values compared to $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$ when $\mathrm{per_{chg}}$ is small, e.g., if $\mathrm{per_{chg}}\leq 20\%$,  $\mathrm{P_{col}}\big(\overline{\mathbf{R}}(\emptyset,\emptyset, \mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R})))\big)\geq 0.92$. Combining Table \ref{table:correlation_attack_compare}, \ref{table:atk_rnd}, and Figure \ref{fig:atkcol_vs_atkrnd}, we conclude that $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$ is not only more powerful (in terms of distorting the fingerprint bit-string), but it also preserves more database utility compared to $\mathrm{Atk_{rnd}}$. % with generating pirated databases.
{\color{black}In addition to the generic utility metrics defined in Section \ref{sec:utility_metrics}, we also calculate and compare the utility some specific statistical computations on the pirated database. For example, under the same attack performance (i.e., compromising exactly 63 fingerprinting bits) $\mathrm{Atk_{col}}(\mathcal{J})$ only causes $0.3\%$ change in the frequency of individuals   having bachelor degree or higher and $0.01$ change for the standard deviation of individuals' age, whereas, the same values for $\mathrm{Atk_{rnd}}$ are $1.4\%$ and $0.12$, respectively. }






\noindent\textbf{Impact of $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$.} 
% {on fingerprint robustness and database utility.}
{\color{black}By setting the threshold $\tau_{\mathrm{row}}^{\mathrm{Atk}} = 0.1$ when comparing $\textstyle\sum_{j\neq i}^{n_c}|s_{ij}^{\mathrm{comm}_c}-\widetilde{s_{ij}}^{\mathrm{comm}_c}|$ in Section \ref{sec:row-wise-atack}} 
we show the impact of $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$ in the blue cells of  Table \ref{table:correlation_attack_compare}. After launching  row-wise correlation attack on $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$, 78 fingerprint bits are distorted at the cost of only $2.9\%$ utility loss. It makes the malicious SP only rank top $82.9\%$ accusable, and may cause Alice accuse innocent SP with high probability.  
% As a result,  $\overline{\mathbf{R}}(\emptyset,\mathrm{Atk_{col}}(\mathcal{S}(\mathbf{R})),\emptyset)$   achieves higher utilities than $\overline{\mathbf{R}}(\emptyset,\emptyset,\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R})))$. 
In particular, we   have  $\mathrm{P_{col}}\big(\overline{\mathbf{R}}(\emptyset,\mathrm{Atk_{col}}(\mathcal{S}(\mathbf{R})),\emptyset)\big) = 0.90$, $\mathrm{P_{row}}\big(\overline{\mathbf{R}}(\emptyset, \mathrm{Atk_{col}}(\mathcal{S}(\mathbf{R})),\emptyset)\big)= 0.95$, and $\mathrm{P_{cov}}\big(\overline{\mathbf{R}}(\emptyset,\mathrm{Atk_{col}}(\mathcal{S}(\mathbf{R})),\emptyset)\big)= 0.97$, which are all closer to that of  $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$. This suggests again that the identified correlation attacks are powerful than the  conventional attacks and they can maintain the utility of database. 




\noindent\textbf{Impact of integrated  correlation attack.} 
% Since $\mathrm{Atk_{row}}(\mathcal{S},C)$ is computationally light and only changes a limited fraction of entries (approximately $1/\gamma$) in $\widetilde{\mathbf{R}}(\mathrm{FP})$, in the integrated attack, we consider that the malicious SP launches $\mathrm{Atk_{row}}(\mathcal{S},C)$ followed by $\mathrm{Atk_{col}}(\mathbb{J})$ and illegally leaks $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\mathrm{Atk_{row}}(\mathcal{S},C),\mathrm{Atk_{col}}(\mathbb{J})\Big)$. In the row- and column-wise correlation attacks, the malicious SP leaks $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\mathrm{Atk_{row}}(\mathcal{S},C)\Big)$ and $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\mathrm{Atk_{col}}(\mathbb{J})\Big)$, respectively. 
% In Table \ref{table:correlation_attack_compare}, we 
% compare the attack performance   (i.e.,  $\mathrm{num_{cmp}}$ and  
%  $r$) and utility loss of the malicious SP (fraction of modified entries as a result of the attack, i.e.,  $\mathrm{per_{chg}} = 1-Acc(\overline{\mathbf{R}})$) 
%  of different correlation attacks 
%  on the vanilla fingerprinted Census database. We observed that by launching the integrated attack, i.e.,    $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$ followed by 8 rounds of $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$,\footnote{It takes 8 while loops for Algorithm \ref{Algo:col-wise-attack} to converge;  the accumulative highly suspicious position set $\mathcal{Z}$ not including new highly suspicious row index and attribute tuple any more. We always let Algorithm \ref{Algo:col-wise-attack} converge when applying $\mathrm{Atk_{col}}(\mathcal{J})$.} the malicious SP   compromises 83 fingerprint bits (out of 128) and causes Alice to accuse $93.72\%$ innocent SPs  (cells highlighted in red in   Table \ref{table:correlation_attack_compare}), with the cost of  only  changing $14.2\%$   entries in $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$. 
%  \hl{EA: also introduce this 128 in the evaluation settings (is there any reason why we picked it this way? should we try higher or smaller values?)}), 
% This suggests that the vanilla fingerprint scheme is not capable of identifying the guilty SP that is liable for the 
% illegal  redistribution of  the database if the malicious SP utilizes correlations in the database to distort the fingerprint. %\hl{EA: will you mention the cost of this attack to the malicious SP in terms of malicious SP's utility as a result of this attack? Even if you will do it later, briefly mention here and refer to later.} 
% If the malicious SP only uses the row-wise correlation and launches $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$ on $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$, it can compromise 78 fingerprint bits  and cause the database owner accuse $82.93\%$ innocent SPs at the cost of only changing $2.9\%$ entries (cells highlighted in  blue). 
% On the other hand, if the malicious SP only conducts $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$, then, at the end of 8 rounds, it is able to compromise 83 fingerprint bits and causes Alice to accuse $91.44\%$ innocent SPs (cells highlighted in green). 
% Although $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$ has similar attack performance compared to the integrated attack, its cost is higher, i.e., $27.1\%$ entries are modified by the attacker. 
% \hl{EA: this reason this is very close to the performance of the integrated attack is the low row-wise correlations? we should comment on this.} 
% Besides, at the early stages of $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$, the malicious SP cannot distort more than half of the fingerprint bits (e.g., at the end of the $5$th round, only 63 bits are compromised by modifying $15.9\%$ of the entries), which is inadequate to cause Alice accuse innocent SPs with probability large than $1\%$.  Since $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$ can distort sufficient  fingerprint bits and cause Alice to accuse innocent SPs with higher probability at a much lower cost of modified data entries, we conclude that it is more powerful than $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$. Next, we investigate the impact of the identified attacks on  fingerprint robustness and database utility separately. 
By launching \\$\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$ on $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$ followed by 8 rounds of $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$, the integrated correlation attack can   distort more fingerprint bits, i.e., 83 bits, which makes the malicious SP's accusable ranking drops to top $93.7\%$ (the cells highlighted in red in Table \ref{table:correlation_attack_compare}). This suggests again that the vanilla fingerprint scheme is not capable of identifying the guilty SP that is liable for pirating the database if the malicious SP utilizes data correlations  to distort the fingerprint.



Note that, although $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$ has similar attack performance compared to the integrated attack, its utility loss is higher, i.e., $27.1\%$ entries are modified by the attacker. Besides, at the early stages of $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$, the malicious SP cannot distort more than half of the fingerprint bits (e.g., at the end of the $5$th round, only 63 bits are compromised by modifying $15.9\%$ of the entries), which is inadequate to cause Alice accuse innocent SPs and also makes the malicious SP uniquely accusable.  Since $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$ can distort sufficient  fingerprint bits and cause Alice to accuse innocent SPs with high probability at a much lower utility loss {\color{black}(measured using both generic utility metrics and specific statistical utilities, like the change in frequencies of data records and standard deviations)}, we conclude that it is more powerful than $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$. {\color{black}This suggests that in real-world integrated correlation attacks, the malicious SP can   conduct $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$  followed by a few rounds of $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$ to simultaneously distort a large number of fingerprint bits and preserve data utility when generating the pirated database.}





\subsubsection{Performance of Mitigation Techniques on Census Database} \label{sec:exp_defense_on_census}


% In the previous section, 
We have shown that correlation attacks can distort the fingerprint bit-string and may make the database owner accuse innocent SPs by resulting in low degradation in terms of database utility. In this section, we first evaluate the proposed mitigation techniques against correlation attacks  separately, and then  consider the integrated  mitigation technique  against the integrated correlation attack, i.e., the row-wise correlation attack followed by the column-wise correlation attack. 
In this experiment, we also assume that Alice  has  access to $\mathcal{S}'$ and $\mathcal{J}'$that  are directly computed from $\mathbf{R}$. Thus, we represent her prior knowledge as  $\mathcal{S}'(\mathbf{R})$ and $\mathcal{J}'(\mathbf{R})$.  As a result, we have $\mathcal{S}' = \mathcal{S}$ and $\mathcal{J}' = \mathcal{J}$. 

% We will study the case of asymmetric prior knowledge in Section \ref{sec:knowledge_asym}. 

% We will also investigate the defense performance of $\mathrm{Dfs_{col}}\mathcal{J}'(\mathbf{R})$ against $\mathrm{Atk_{col}}\mathcal{J}(\mathbf{R})$ that utilizing  higher order of column-wise correlations in Appendix \ref{sec:higher_order}.


\noindent\textbf{Performance of $\mathrm{Dfs_{col}}(\mathcal{J}'(\mathbf{R}))$.} As discussed in Section \ref{sec:col_defense}, the mitigation strategy is determined by the marginal probability mass transportation plan, which is heterogeneous for higher $\lambda_p$ (a tuning parameter controlling the entropy of the transportation plan) and homogeneous for lower $\lambda_p$. To evaluate the utility loss due to $\mathrm{Dfs_{col}}(\mathcal{J}'(\mathbf{R}))$, we calculate the utility of  $\widetilde{\mathbf{R}}\big(\mathrm{FP},\emptyset,\mathrm{Dfs_{col}}(\mathcal{J}'(\mathbf{R}))\big)$ by setting $\lambda_p   \in \{100,\cdots,1000\},\forall p\in\mathcal{F}$, and show 
the results in Figure \ref{fig:utility_lambda}. We see that all utilities monotonically increase as the mass transportation plans transform from homogeneous to heterogeneous (i.e., as $\lambda_p$ increases). This is because, as the transportation plans become more heterogeneous, the mitigation technique can tolerate more discrepancy between two marginal distributions (Section \ref{sec:col_defense}), and hence fewer number of entries are modified by $\mathrm{Dfs_{col}}(\mathcal{J}'(\mathbf{R}))$.




\begin{figure}[htb]
  \begin{center}
     \includegraphics[width= 0.6\columnwidth]{figures/utility_lambda-eps-converted-to.pdf}
      \end{center}
  \caption{\label{fig:utility_lambda} Utilities of $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\mathrm{Dfs_{col}}(\mathcal{J}'(\mathbf{R})))$ under varying $\lambda_p$.}
\end{figure}


Next, we fix $\lambda_p  = 500, \forall p\in\mathcal{F}$,   evaluate the performance (in terms of both fingerprint  robustness and database utility) of launching $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$  on $\widetilde{\mathbf{R}}\big(\mathrm{FP},\emptyset,\mathrm{Dfs_{col}}(\mathcal{J}'(\mathbf{R}))\big)$ with increasing attack rounds. In Figure \ref{fig:atkcol_after_dfscol}(a), we observe that at then end of 8 rounds of $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$, the malicious SP can only compromise 24 (out of 128) fingerprint bits, which is not enough to cause Alice accuse innocent SPs and will make itself uniquely accusable.   In contrast, as shown in Table \ref{table:correlation_attack_compare}, when launching $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$ on the vanilla fingerprinted database $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$, the malicious SP can compromise 82 bits and make itself only rank top $91.4\%$ accusable.  This suggests that proposed $\mathrm{Dfs_{col}}(\mathcal{J}'(\mathbf{R}))$ significantly mitigates the column-wise correlation attack. 



\begin{figure}[htb]
  \begin{center}
  \begin{tabular}{cc}
     \includegraphics[width= .4\columnwidth]{figures/fp_robust_atkcol_after_dfscol-eps-converted-to.pdf}
		&
		     \includegraphics[width= .4\columnwidth]{figures/db_utility_atkcol_after_dfscol-eps-converted-to.pdf}
 \\
    {\small  (a) Fingerprinting robustness}  &
    {\small  (b) Database utilities} \\
    {for increasing attack rounds.} &
     {for increasing attack rounds.} \\
        \end{tabular}
      \end{center}
  \caption{\label{fig:atkcol_after_dfscol} Fingerprint robustness and database utilities when launching $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R})))$ on $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\mathrm{Dfs_{col}}(\mathcal{J}'(\mathbf{R})))$.}
\end{figure}


Furthermore, in Figure \ref{fig:atkcol_after_dfscol}(b) we observe that $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$ also degrades the utilities of the vanilla fingerprinted database post-processed by $\mathrm{Dfs_{col}}(\mathcal{J}'(\mathbf{R}))$. In particular, the accuracy drops to 0.76 and the preservation of column-wise correlation drops to 0.67 at the end of 8 rounds of $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$. Combining  Figures \ref{fig:utility_lambda} and \ref{fig:atkcol_after_dfscol}, we conclude that, as a post-processing step, the proposed column-wise correlation mitigation technique provides robust fingerprint against column-wise correlation attack and preserves   database utility. 



\noindent\textbf{Performance of $\mathrm{Dfs_{row}}(\mathcal{S}'(\mathbf{R}))$.} In Table \ref{table:performance-row-defense}, we evaluate the performance of the robust fingerprinted database against row-wise attack, i.e., $\widetilde{\mathbf{R}}(\mathrm{FP},\mathrm{Dfs_{row}}(\mathcal{S}'(\mathbf{R}),\emptyset)$, along with the pirated database obtained by launching $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R})$ on it. Clearly, $\mathrm{Dfs_{row}}(\mathcal{S}'(\mathbf{R}))$ successfully defends against $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$, since the pirated database only distorts 13 fingerprint bits and makes the malicious SP uniquely accusable. Combining this result with Table \ref{table:correlation_attack_compare} (cells in blue), we conclude that $\mathrm{Dfs_{row}}(\mathcal{S}'(\mathbf{R}))$ not only mitigates the row-wise correlation attack but it also preserves the database utility. 

\begin{table}[htb]
\begin{center}
 \begin{tabular}{c | c|c| c | c | c| c } 
 \hline
 \hline
  &    $Acc$ &  $\mathrm{P_{col}}$  & $\mathrm{P_{row}}$ & $\mathrm{P_{cov}}$ & $\mathrm{num_{cmp}}$ &  $r$ \\
 \hline
$\widetilde{\mathbf{R}}(\mathrm{FP},\mathrm{Dfs_{row}}(\mathcal{S}'),\emptyset)$  &  0.97    & 0.94   & 0.99  &  0.99 & N/A  &   N/A \\ 
$\overline{\mathbf{R}}(\emptyset,\mathrm{Atk_{row}}(\mathcal{S}),\emptyset)$ &    0.93 & 0.92  & 0.94& 0.98 & 13& u  \\
  \hline
  \hline
\end{tabular}
\caption{Impact of  $\mathrm{Dfs_{row}}(\mathcal{S}'(\mathbf{R}))$ before and after $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$. $r=\text{u}$ means uniquely accusable.} 
\label{table:performance-row-defense}
\end{center}
\end{table}


\noindent\textbf{Performance of integrated mitigation.} Here, we investigate the performance of the integrated mitigation  against the integrated correlation attacks. By setting $\lambda_p=500, \forall p \in \mathcal{F}$, we evaluate the utility of $\widetilde{\mathbf{R}}\big(\mathrm{FP},\mathrm{Dfs_{row}}(\mathcal{S}'(\mathbf{R})),\mathrm{Dfs_{col}}(\mathcal{J}'(\mathbf{R}))\big)$ before and after it is subject to the integrated attack, i.e.,  $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$ followed by $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$. We show the results in Table \ref{table:int-dfs-int-atk}. Clearly,  after   integrated mitigation, the fingerprinted database still maintains high utilities. Even if the malicious SP launches  integrated correlation attack, it can only compromise 4 fingerprint bits and  makes itself uniquely accusable. It suggests that the proposed mitigation techniques provide high robustness against integrated correlated attacks. 
 

\begin{table}[htb]
\begin{center}
% \resizebox{0.78\textwidth}{!}{\begin{minipage}{\textwidth}
 \begin{tabular}{c | c|c| c | c | c| c } 
 \hline
 \hline
  &    $Acc$ &  $\mathrm{P_{col}}$  & $\mathrm{P_{row}}$ & $\mathrm{P_{cov}}$ & $\mathrm{num_{cmp}}$ &  $r$ \\
 \hline
% $\widetilde{\mathbf{R}}(\mathrm{FP},\mathrm{Dfs_{row}}(\mathcal{S}'(\mathbf{R})),\mathrm{Dfs_{col}}(\mathcal{J}'(\mathbf{R})))$  
after int. mitigation&  0.94    & 0.91   & 0.96  &  0.97 & N/A  &   N/A \\ 
% $\overline{\mathbf{R}}(\emptyset,\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R})),\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R})))$ 
after int. attack&    0.77 & 0.82  & 0.86 & 0.94 & 4& u \\
  \hline
  \hline
\end{tabular}
% \end{minipage}}
\caption{Impact of  integrated mitigation    before and after   integrated correlation attack. $r=\text{u}$ means uniquely accusable.} 
\label{table:int-dfs-int-atk}
\end{center}
\end{table}



% \vspace{-2mm}
% \subsubsection{Validation of   Theoretical Analysis on the Identified Correlation Attacks}
% \label{sec:theory_validate}
% {\color{black}Here, given different fingerprinting ratio $\gamma$, we investigate the malicious SP's confidence gain, i.e.,  $G_{\mathrm{col}}(\frac{1}{\gamma};p,a)$ and $G_{\mathrm{row}}(\frac{1}{\gamma};\boldsymbol{r}_i)$ (introduced in Sections \ref{sec:col-wise-attack} and \ref{sec:row-wise-atack}). For this experiment, we let $p$ be the attribute of ``age" and $a=3$ (after encoding).}


% \begin{figure}[htb]
%   \begin{center}
%   \begin{tabular}{cc}
%      \includegraphics[width= .45\columnwidth]{figures/conf_gain_column.eps}
% 		&
% 		     \includegraphics[width= .45\columnwidth]{figures/conf_gain_row.eps}
%  \\
%     {\small  (a) SP's confidence gain that an}  &
%     {\small  (b) SP's confidence gain that a} \\
%     {entry whose attribute $p$ is $a$ is} &
%      {particular entry $\boldsymbol{r}_i$ is} \\
%      {fingerprinted under varying $\frac{1}{\gamma}$.}&
%      {fingerprinted under varying $\frac{1}{\gamma}$.}
%         \end{tabular}
%       \end{center}
%   \caption{\label{fig:conf_gain} Evaluation of the confidence gain of fingerprinting under different correlation attacks with and without the corresponding mitigation techniques.}
%   \vspace{-3mm}
% \end{figure}



% {\color{black} In Figures \ref{fig:conf_gain}(a) and (b), we show the theoretical values of $G_{\mathrm{col}}(\frac{1}{\gamma};p,a)$ and $G_{\mathrm{row}}(\frac{1}{\gamma};\boldsymbol{r}_i)$ under varying $\frac{1}{\gamma}$, and compare these with the empirical values obtained after the correlation attacks without (black curves) and with (red curves) the corresponding mitigation techniques. The empirical values of $G_{\mathrm{col}}(\frac{1}{\gamma};p,a)$ and $G_{\mathrm{row}}(\frac{1}{\gamma};\boldsymbol{r}_i)$ are calculated as the frequency of the entries whose attribute $p$ takes value $a$ is fingerprinted in the constructed suspicious set $\mathcal{P}$, and the frequency of rows identified as fingerprinted by $\mathrm{Atk_{row}}(\mathcal{S})$, respectively. We observe that the confidence gain after the mitigation techniques is always smaller than that the one without the mitigation techniques, and is close to $1$ when the fingerprint ratio is high, i.e., $\frac{1}{\gamma}$ is small. The experiment results are consistent with our theoretical findings in Proposition \ref{prop:atk_col} and \ref{prop:atk-row}, and validate the effectiveness of the developed mitigation techniques by showing that the the proposed mitigation techniques make the confidence gain of a malicious SP only sightly better than $\mathrm{Atk_{rnd}}$. The gaps between the blue curves (theoretical values) and black curves are due to the applying of inequalities during derivations. Please refer to   Appendix \ref{sec:supp_algos_col-wise-attack} and \ref{sec:supp_algos_row-wise-attack} for details.

% }
 
% \subsubsection{Investigation  of   Asymmetric Prior Knowledge}
% \label{sec:knowledge_asym}


% As discussed in Section \ref{sec:system-threat}, to   the advantage of the malicious SP, we assume that the malicious SP has more accurate or at least equally accurate knowledge (compared to the database owner Alice) about row-wise and column-wise correlations in the database. 
% Thus, in the following, we investigate the scenario, in which the malicious SP uses the accurate knowledge, whereas Alice uses inaccurate prior knowledge to implement the proposed mitigation techniques.  {\color{black}Due to the space limit, we only highlight the empirical findings here, i.e.,   the proposed mitigation techniques with inaccurate knowledge can alleviate the correlation attacks even if the malicious SP has access to accurate correlations. Please refer to Appendix \ref{sec:inaccurate_atk} for the setups and results for this experiment.}






% We also provide experiments evaluating the opposite case in Appendix \ref{sec:inaccurate_atk}. 
% To generate inaccurate  column- and row-wise correlations, we assume Alice's knowledge on  $\mathcal{J}'$ and $\mathcal{S}'$ is computes from $\mathbf{R}_\kappa$, which is obtained by randomly removing $\kappa$ percentage of data records from $\mathbf{R}$. We represent the mitigation techniques using inaccurate knowledge as $\mathrm{Dfs_{col}}(\mathcal{J}'(\mathbf{R}_\kappa))$ and $\mathrm{Dfs_{row}}(\mathcal{S}'(\mathbf{R}_\kappa))$.


% \begin{figure*}[htb]
%   \begin{center}
%   \begin{tabular}{ccccc}
%      \includegraphics[width= .38\columnwidth, height=1.8cm]{figures/asy_noisy_col_dfs_fp_robust.eps}
% 		&
% 		     \includegraphics[width= .38\columnwidth, height=1.8cm]{figures/asy_noisy_col_dfs_acc.eps}
% 		&
%      \includegraphics[width= .38\columnwidth, height=1.8cm]{figures/asy_noisy_col_dfs_p_col.eps}
%      		&
%      \includegraphics[width= .38\columnwidth, height=1.8cm]{figures/asy_noisy_col_dfs_p_row.eps}
%           		&
%      \includegraphics[width= .38\columnwidth, height=1.8cm]{figures/asy_noisy_col_dfs_cov.eps}
%      \\
%     {\small  (a) robustness}  &
%     {\small  (b) $Acc$} &
%     {\small  (c) $\mathrm{P_{col}}$} &
%     {\small  (d) $\mathrm{P_{row}}$} &
%     {\small  (e) $\mathrm{P_{cov}}$}\\
%         \end{tabular}
%       \end{center}
%   \caption{\label{fig:noisy_dfs_col}  Evaluation of fingerprint robustness and database utility considering $\mathrm{Dfs_{col}}(\mathcal{J}'(\mathbf{R}_\kappa))$ and $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$.}
% \end{figure*}




% \begin{figure*}[htb]
%   \begin{center}
%   \begin{tabular}{ccccc}
%      \includegraphics[width= .38\columnwidth, height=1.8cm]{figures/asy_noisy_row_dfs_fp_robust.eps}
% 		&
% 		     \includegraphics[width= .38\columnwidth, height=1.8cm]{figures/asy_noisy_row_dfs_acc.eps}
% 		&
%      \includegraphics[width= .38\columnwidth, height=1.8cm]{figures/asy_noisy_row_dfs_p_col.eps}
%      		&
%      \includegraphics[width= .38\columnwidth, height=1.8cm]{figures/asy_noisy_row_dfs_p_row.eps}
%           		&
%      \includegraphics[width= .38\columnwidth, height=1.8cm]{figures/asy_noisy_row_dfs_cov.eps}
%      \\
%     {\small  (a) robustness}  &
%     {\small  (b) $Acc$} &
%     {\small  (c) $\mathrm{P_{col}}$} &
%     {\small  (d) $\mathrm{P_{row}}$} &
%     {\small  (e) $\mathrm{P_{cov}}$}\\
%         \end{tabular}
%       \end{center}
%   \caption{\label{fig:noisy_dfs_row}  Evaluation of fingerprint robustness and database utility considering $\mathrm{Dfs_{row}}(\mathcal{S}'(\mathbf{R}_\kappa))$ and $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$.}
% \end{figure*}






% \noindent\textbf{Scenario 1: $\mathrm{Dfs_{col}}(\mathcal{J}'(\mathbf{R}_\kappa))$  vs. $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$.} By varying $\kappa$ from 1 to 15, we evaluate  the fingerprint robustness and database utility before and after $\widetilde{\mathbf{R}}\big(\mathrm{FP},\emptyset,\mathrm{Dfs_{col}}(\mathcal{J}'(\mathbf{R}_\kappa))\big)$ is attacked by $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$, and show the results in Figure \ref{fig:noisy_dfs_col}. 
% In particular, Figure \ref{fig:noisy_dfs_col}(a) shows that as $\kappa$ increases, i.e., $\mathcal{J}'(\mathbf{R}_\kappa)$ becomes less accurate, the number of distorted fingerprint bits by the malicious SP increases from 18 to 35, however, even for the most inaccurate $\mathcal{J}'(\mathbf{R}_\kappa)$ (when $\kappa=15$), we observer that the malicious SP cannot distort more than half of the fingerprint bits, and thus it will be uniquely accusable. 
% Figure \ref{fig:noisy_dfs_col}(b)-(e) compare different utility metrics of $\widetilde{\mathbf{R}}\big(\mathrm{FP},\emptyset,\mathrm{Dfs_{col}}(\mathcal{J}'(\mathbf{R}_\kappa))\big)$ and that attacked by $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$, i.e., $\overline{\mathbf{R}}(\emptyset,\emptyset,\mathrm{Atk_{col}}(\mathbf{R}))$. 
% We observe that even with inaccurate column-wise correlations, Alice can still achieve high utilities when generating the robust fingerprinted database. If the malicious SP attacks using the accurate column-wise correlations, it causes large utility losses in the pirated database, i.e., $Acc$ drops to $0.758$ when $\kappa=15$. This experiment validates that the proposed column-wise mitigation technique is robust even with inaccurate knowledge of the database owner. 






% \noindent\textbf{Scenario 2: $\mathrm{Dfs_{row}}(\mathcal{S}'(\mathbf{R}_\kappa))$  vs. $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$.} In Figure \ref{fig:noisy_dfs_row}, we show the   experiment results when $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\mathrm{Dfs_{row}}(\mathcal{S}'(\mathbf{R}_\kappa)),\emptyset\Big)$  is subject to $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$. Similar to before, as $\mathrm{Dfs_{row}}(\mathcal{S}'(\mathbf{R}_\kappa))$ becomes less accurate, the malicious SP can distort more fingerprint bits by launching $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$. However, as shown in Figure \ref{fig:noisy_dfs_row}(a), it is still unable to distort more than half of the bits to avoid being identified by Alice. Furthermore, Figure \ref{fig:noisy_dfs_row}(b)-(e) show that row-wise mitigation technique with inaccurate knowledge still preserves database utilities. 
% These results corroborate that the proposed mitigation techniques with inaccurate knowledge can alleviate the correlation attacks even if the malicious SP has access to   accurate correlations.  







% \begin{table*}[htb]
% \begin{center}
%  \begin{tabular}{c | c|c| c | c | c| c| c| c| c| c} 
%  \hline
%  \hline
% \multirow{2}{*}{$\mathrm{Dfs_{col}}\Big(  \mathbb{M}(\mathbf{R},\kappa)  , \mathbb{J}(\mathbf{R},\kappa) \Big)$}& cumulative KL &changed & \multicolumn{8}{c}{Attacking rounds of $\mathrm{Atk_{col}}\Big(  \mathbb{M}(\mathbf{R})  , \mathbb{J}(\mathbf{R}) \Big) $ after $\mathrm{Dfs_{col}}\Big(  \mathbb{M}(\mathbf{R},\kappa)  , \mathbb{J}(\mathbf{R},\kappa) \Big)$  }\\
% \cline{4-11}
% &   divergence  &entries (\%)   & 1&2&3&4&5&6&7&8 \\
%  \hline
%  \rowcolor{Gray}
%          $\kappa=0$&   100  &  85 &   73   & 70   & 65   & 54 &   51  &  46 \\ 
% (noise free)& 0   &      0   &      0  &  0.0800 &   0.7300 &  53.2100  & 71.8300 &  91.4400 \\
%   \hline
% $\sigma$& 102&  83  &71 & 69 &66&55  &  49   & 48  \\ 
% $=2\times 10^{-4}$& 0    &     0 &   0.0900 &   0.2900  &  0.9700   &45.9200 &  81.2700 &  90.2700 \\
%   \hline
%   $\sigma$& 103  &  87   & 75  &  70  &  67  &  52  &  49  &  48 \\ 
% $=4\times 10^{-4}$& 0      &    0     &     0    & 0.0700   &  0.3900   & 49.3300   & 72.4200  &  83.6000\\
%   \hline
%     $\sigma$&  103  &  85  &  78   & 75   & 72  &  55 &   52   & 51  \\ 
% $=6\times 10^{-4}$&0      &   0      &   0    &     0     &    0  & 26.8100 &  65.0400 &  72.4600 \\
%   \hline
%       $\sigma$&   105  &  90   & 80  &  77  &  77   & 59  &  59  &  57  \\ 
% $=8\times 10^{-4}$&0      &   0    &     0     &    0       &  0  & 14.1500  & 14.1500&   27.5500 \\
%   \hline
%       $\sigma$&    107   & 89   & 83  &  82 &   81    &70 &   68 &   65  \\ 
% $=10\times 10^{-4}$& 0     &    0        & 0     &    0      &   0  &  0.1500  &  0.4100 &   3.1800 \\
%   \hline
%  \hline
% \end{tabular}
% \caption{$\mathrm{Dfs_{col}}(  \mathbb{M}(\mathbf{R},\kappa)  , \mathbb{J}(\mathbf{R},\kappa) )$.} 
% \label{table_notations}
% \end{center}
% \end{table*}




























 





% \subsection{Evaluations on Genome Database}
% \label{sec:geo_experiment}
% We also evaluate the identified attacks and proposed robust fingerprinting schemes on a genome relational database. We use genome data belonging to 1000 individuals from the HapMap dataset~\cite{gibbs2003international}. 
% Each individual has $156$ data points (i.e.,mutations) represented as single-nucleotide polymorphisms (SNPs). A SNP is a point mutation on the DNA and it is represented by its number of minor alleles (i.e., the nucleotide, which is observed in the minority of the population). Also, each SNP includes 2 alleles (nucleotides), and hence value of a SNP is typically represented as 0, 1, or 2. 
% %we first consider 1000 individuals, each of which is characterized by a sequence of genome   with length 156~\cite{gibbs2003international}. Each genome data point is represented by the number of minor alleles (i.e., the nucleotide which is observed in the minority of the population) at a specific single-nucleotide polymorphism (SNP) position. Since each person can have either 0, 1, or 2 minor alleles at a SNP position, the genome data of each individuals is in the support of $\{0,1,2\}^{1\times 156}$. 
% Each nucleotide of a SNP is inherited from a parent, and hence genomes of family members are correlated. To observe the effect of row-wise correlations in the genome dataset, we create synthetic family members in the dataset. For this, we randomly split the 1000 individuals into 500 mother and father pairs and apply the Mendel's law to generate the genome data of their (synthetic) children. %(refer to Appendix~\ref{sec:tou_mendel} for an example).  
% As a result, we obtain a genome relational database with 1500 individuals (rows) each having 156 attributes (columns). %Please refer to Appendix~\ref{sec:tou_mendel} for an example of generating a child's genome data using the Mendel's law. 
% In this experiment, we assume that both the database owner (Alice) and the malicious SP have access to data correlations that are directly computed from the original genome database and they also know about (i) the communities (i.e., families) in the database and (ii) the Mendel's law. 

% %It is noteworthy that all considered schemes (i.e., fingerprinting, attacks, and mitigation techniques) need to avoid introducing biologically impossible entries when modifying the genome data points.\footnote{Considering a SNP at a specific position, if both mother and father has 0 minor allele at that position, then their child will also have 0 minor allele at the same position. If either mother or father has 0 minor allele and the other has 2 minor allele, then their child must have 1 minor allele at that position. If a applied scheme generates data points that violates the above situation, the users (Alice or the malicious SP) needs to change it to a biologically possible one.} 





% \subsubsection{Impact of Correlation Attacks on Genome Database}
% In Table \ref{table:genome-all-attacks} in Appendix~\ref{sec:gen_result}, we show the experiment results on the utility and fingerprint robustness when the vanilla fingerprinted genome database $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$ is subject to the random bit flipping attack and the identified correlation attacks. 
% As expected, $\mathrm{Atk_{rnd}}$ has the weakest attacking performance; even if we let the malicious SP change half of the entries (i.e., $Acc(\overline{\mathbf{R}}(\mathrm{Atk_{rnd}},\emptyset,\emptyset)) = 0.5$), it still cannot distort any fingerprint bits, and hence render the malicious SP uniquely accusable. 
% We observe that $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$ not only preserves the database utility, but it also has the best attack performance; it distorts 104 (out of 128) fingerprint bits and help the malicious SP avoid the accuse. The malicious SP ranks only top 100\% accusable, which suggest that Alice will accuse an innocent SP almost certainly. 
% The reason is that the communities among the individuals are determined by the kinship and each community only has 3 individuals, which suggests that the row-wise statistical relationships are strong, and if the malicious SP has access to $\mathcal{J}(\mathbf{R})$, it can identify most of the fingerprinted entries. 
% Compared with $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$, $\mathrm{Atk_{col}}(\mathcal{J}(\mathbf{R}))$ (with 11 attacking rounds) only distorts 7 fingerprint bits by changing $3\%$ of the entries and also makes the malicious SP uniquely accusable. This is because the considered genome database has significantly more attributes than the Census database, hence it is difficult for $\mathrm{Atk_{col}}(\mathcal{S}(\mathbf{R}))$ to locate the exact fingerprinted position, i.e., identify the correct suspicious tuple $\{i,p\}\in\mathcal{P}$. As a consequence, the integrated correlation attack also gives a similar attack performance as $\mathrm{Atk_{row}}(\mathcal{S}(\mathbf{R}))$. 
 
 
 
 





% \subsubsection{Performance of Mitigation Techniques on Genome Database}

% In Table~\ref{table:genome-all-defense} in Appendix~\ref{sec:gen_result}, we show the performance of different mitigation techniques against the corresponding correlation attacks. We observe that all mitigation techniques preserve high database utility and they significantly alleviate the correlation attacks. Thus, the malicious SP becomes uniquely accusable even if it considers the data correlations in its attacks. This also shows that the proposed mitigation techniques can be applied for robust fingerprinting of databases with different types of correlated data. 








==> sections/introduction.tex <==



% \hl{TJ: do we need to include CCS concepts and keywords?}

\section{Introduction}


% In recent decades, gigantic amounts of data have been generated at a unprecedented rate  from a variety of sources, and  
% Relational databases (or relations) have become the most popular database systems ever since 1970s. A relation is defined as a set of data records  that have the same attributes  
% % , and each row is identified by a unique key~
% \cite{codd2002relational}. 
% Constructing and sharing of the relations are   critical to the vision of a data-driven future 
% %with convenient lifestyles 
% that benefit all human-beings. For example, individuals  can enjoy customized services offered by \emph{service providers} (SPs), such as 
% % Netflix for personalized movie recommendations, 
% outsourced computation by Amazon Elastic Compute Cloud and    recreational genomic services by 23andme \cite{site:23andme}  through sharing their private data with SPs. 
% % On the other hand, to receive such customized services, individuals need to pay in terms of the bits and bytes of their personal data, and hence their privacy. 
% Most of the time, sharing such information with a particular SP is done via consent of an individual, and the collected personal data in the relational databases is shared with other (authorized) parties for various purposes, including personal advertisements or research. 


% However, when such relational databases are shared or leaked beyond the authorized SPs (who are authorized to receive/use the database), individuals' privacy is violated. 
% As a consequence, preventing unauthorized sharing of databases is of great importance. 
% Database owners (who collect data from individuals and construct the dataset) want to (i) make sure that shared data is used only by the authorized parties for specified purposes and (ii) discourage such parties from releasing the received datasets to other unauthorized third parties (either intentionally or unintentionally). Such data breaches cause financial and reputational damage to database owners. Therefore, identifying the source of data breaches is crucial for database owners to hold the identified party responsible.


Relational databases (or relations) have become the most popular database systems ever since 1970s. A relation is defined as a set of data records  with the same attributes~\cite{codd2002relational}. 
Constructing and sharing of the relations are critical to the vision of a data-driven future that benefits all human-beings. {\color{black}It   supports broader range of tasks in real-life than just sharing database statistics or  machine learning models trained from the database.} 
For example, a relational database owner (who collects data from individuals and constructs the dataset) can benefit from outsourced computation (e.g., from service providers (SP) like Amazon Elastic Compute Cloud), let other SPs analyze its data  (e.g., for personal advertisements), or  exchange datasets for collaborative research after data use agreements.



% share its database with other SPs for research. 
%For example, a relational database owner (who collects data from individuals and constructs the dataset) can enjoy customized services offered by \emph{service providers} (SPs), e.g., outsourced computation by Amazon Elastic Compute Cloud and recreational genomic services by 23andme \cite{site:23andme} through sharing her database with SPs. 


Most of the time, sharing a database with an authorized  SP (who is authorized to receive/use the database) is done via consent of the database owner. However, when such   databases are shared or leaked beyond the authorized SPs, individuals' (people who contribute their data in the  database) privacy is violated, and hence preventing unauthorized sharing of databases is of great importance. Thus, database owners want to (i) make sure that shared data is used only by the authorized parties for specified purposes and (ii) discourage such parties from releasing the received datasets to other unauthorized third parties (either intentionally or unintentionally). Such data breaches cause financial and reputational damage to database owners. 
For instance, it is reported that the writing site Wattpad suffered a major data breach in July 2020; over 270 million individuals'  data were sold on a third party   forum in the darknet \cite{Wattpadd66:online}. 
Therefore, identifying the source of data breaches is crucial for database owners to hold the identified party responsible.



 
Digital fingerprinting is a technology that allows to identify the source of data breaches by embedding a unique mark into each shared copy of a digital object. Unlike digital watermarking, in fingerprinting, the embedded mark must be unique to detect the guilty party who is responsible for the leakage. Although the most prominent usage of fingerprinting is in the multimedia domain \cite{cox1997secure,cox2002digital,johnson2001information}, fingerprinting techniques for databases have also been developed \cite{li2005fingerprinting,guo2006fingerprinting,liu2004block,lafaye2008watermill}. These techniques change database entries at different positions when sharing a database copy with a SP. 
However, existing fingerprinting schemes for databases have been developed to embed fingerprints in continuous-valued numerical entries (floating points) in relations. On the other hand, fingerprinting discrete (or categorical) values is more challenging, since the number of possible values (or instances) for a data point is much fewer. Hence, in such databases, a small change in the value of a data point (as a fingerprint) can significantly affect the utility. 
In addition, existing fingerprinting schemes for databases do not consider various inherent correlations between the data records in a database. A malicious party having a fingerprinted copy of a database can detect and distort the embedded fingerprints using its knowledge about the correlations in the data. For example, the zip codes are strongly correlated with street names in a demographic database  making common fingerprinting schemes venerable to attacks utilizing such correlations. Thus,   to provide robustness against correlation attacks (which utilizes the correlations between attributes and data records to infer the potentially fingerprinted entries), we need to consider  such correlations when developing  fingerprinting schemes for relational database. % need to consider such correlations. % in the database.

In this work, we first identify correlation attacks against the existing database fingerprinting schemes. Namely, we present column-wise correlation attack, row-wise correlation attack, and the integration of both. To launch these attacks, a malicious SP utilizes its prior knowledge about correlations  between the columns (attributes) of database, statistical relationships between the rows (data records), and the combination of both.  
After launching these attacks on a fingerprinted database, the malicious SP can easily distort the added fingerprint to mislead the fingerprint extraction algorithm and cause the database owner to accuse innocent parties. For example, we show that by changing $14.2\%$   entries in a database, the integration of row- and column-wise correlation attack can distort $64.8\%$ fingerprint bits and cause the database owner falsely accuse innocent SPs with high probability.  
%{\color{blue}innocent SPs as the percentile of accusing the right malicious SP reduces from 1  to 0.063 (here 1 means accusing with the highest certainty).} 
This suggests that existing database fingerprinting schemes are vulnerable to identified correlation attacks, and mitigation techniques are in dire need. 


To reduce the identified vulnerability in existing database fingerprinting schemes, we propose   novel mitigation techniques  to provide robust fingerprinting   that can alleviate the   correlation attacks. 
Although,   we describe the proposed techniques for a specific vanilla database fingerprinting scheme \cite{li2005fingerprinting}, they can be applied  to other   schemes as well. In other words, the proposed mitigation techniques can work as  post-processing steps for any off-the-shelf database  fingerprinting schemes   and make them robust against potential attacks that utilize the inherent  data correlations. 
The proposed mitigation techniques utilize database owner's prior knowledge on the column- and row-wise correlations. In particular, to mitigate the column-wise correlation attack, the database owner modifies some of the non-fingerprinted data entries to make the post-processed fingerprinted database have column-wise correlations close to that of her prior knowledge. The data entry modification plans are determined from the solutions to a set of ``optimal transportation'' problems~\cite{courty2016optimal}, {\color{black}each of which transports the mass of the marginal distribution of a specific attribute (column) to make it resemble the reference marginal distribution computed from database owner's prior knowledge while minimizing the transportation cost.} 
% which resemble the marginal probability distributions (with respect to the attributes) of the new databases to a set of reference marginal distributions. 
To alleviate the row-wise correlation attack, the database owner modifies limited number of non-fingerprinted data entries by solving a combinatorial search problem to make the post-processed fingerprinted database have row-wise statistical relationships that are far away from that of her prior knowledge. We show that even if the malicious SP has access to  the exactly same prior knowledge (i.e., data correlation models) with the database owner,   the proposed mitigation techniques can effectively reduce the vulnerability caused by correlation attacks. 
The proposed mitigation techniques also maintain the utility of the post-processed fingerprinted database   by (i) encoding the database entries as integers, such that the least significant bit (LSB) carries the least information, and adding the fingerprint by only changing the LSBs; and (ii) changing only a small number of database entries.  


% \ea{Briefly describe the key technical contributions. Especially, mention how the proposed technique mitigates the considered attacks and provides high data utility} 

% To   validate the   effectiveness of the proposed mitigation techniques. We consider two real world relational databases, i.e., a Census database and a genome database. Specifically, we show that 

 

We use an real-world Census relational database to validate the effectiveness of the proposed robust fingerprinting scheme against  the identified correlation attacks.   In particular,  we show that the  malicious SP can only compromise $3\%$ fingerprint bits, even if it launches the powerful integrated correlation attack on the Census database. Thus,  it will   be held as responsible for data leakage.  


We summarize the main contributions of this paper as follows:
\begin{itemize}
  \item We identify correlation attacks 
%   (i.e.,   column-wise correlation attack, row-wise correlation attack, and the integration of them) 
  that can distort large portion of the fingerprint bits in the  existing database fingerprinting scheme and cause the database owner to accuse innocent SPs with high probability.
  \item We propose robust fingerprinting scheme that involves novel mitigation techniques to alleviate the impact of the identified correlation attacks. The proposed mitigation techniques can work as post-processing steps for any off-the-shelf database fingerprinting schemes.
  \item We   investigate the impact of the identified correlation attacks and the proposed mitigation techniques on an real-world relational database. We show that the correlation attacks are more powerful than traditional attacks, because they can  distort more   fingerprint bits with less utility loss. On the other hand,   the  mitigation techniques can effectively alleviate these attacks and maintain database utility even if  the malicious SP   uses data correlation models that are directly calculated from the data.
  
%   database owner’s prior knowledge is less accurate compared to that of the malicious SP. 
\end{itemize}


The rest of this paper is organized as follows.  We review related works on existing fingerprinting schemes in Section \ref{sec:related_work}, which is followed by the description on the considered vanilla fingerprinting scheme in Section \ref{sec:vanilla}. In Section \ref{sec:system-threat}, we present the system and threat models, and evaluation metrics. Section \ref{sec:corr_attacks} introduces the identified correlation attacks. In Section \ref{sec:robust_fp}, we develop   robust fingerprinting against the identified attacks. We evaluate the impact of correlation attacks and the performance of the proposed mitigation techniques in Section \ref{sec:eva}. Finally, Section \ref{sec:conclusion} concludes the paper. 





%In this work, we consider the row index of a record in a relation as its primary key. \ea{I didnt understand what this means}




%\ea{Watermarking or fingerprinting as a potential solution to this problem. Show examples from other domains (multimedia)}

%\ea{Mention the difference of watermarking and fingerprinting}

%Discrete or (and) categorical relations are ubiquitous in real life databases, such as the Census Income database \cite{kohavi1996scaling}, the Breast Cancer database, and the Bach Chorales database \cite{asuncion2007uci}. %However, most of the fingerprinting schemes are developed to embed watermarks in continuous-valued numerical entries (floating points) in relations, e.g.,  \cite{li2005fingerprinting,guo2006fingerprinting,liu2004block,lafaye2008watermill}, and fingerprinting discrete entries has been rarely studied...\ea{cite the existing ones and briefly mention their limitations.} \ey{Fingerprinting discrete values is more challenging since the number of possible values for a data point is much lower and making a small change in the value of a data point as a fingerprint can affect the utility considerably.}


%Necessity of considering correlations among categorical or discrete entries in relational databases. 
%..

%\ea{Mention (and give example about) both column-wise and row-wise correlations}

%...

%\ea{For the above item: such existing fingerprinting schemes are actually proposed for databases, right? Let's make sure this is clear. Here, we identify a vulnerability for such schemes, show this vulnerability, and propose an add-on that would work together with existing fingerprinting mechanism for relational databases.}

%\ea{Discuss the potential attacks the attacker can launch. Should we tell here that collusion is also a potential attack (not considered so for for database fingerprinting) and we will consider it in future work?} 





==> sections/preliminaries.tex <==
%\section{Preliminaries}

\section{The Vanilla Fingerprint Scheme}
\label{sec:vanilla}

In this work, we consider the  fingerprinting scheme proposed in \cite{li2005fingerprinting} as the vanilla scheme, for which we show the vulnerability and develop the proposed scheme.  
% This scheme It extends the watermarking  scheme developed in \cite{agrawal2003watermarking} in a significant way to
% supports the insertion and detection of arbitrary fingerprint bit-string  in databases.  
Assume a database owner shares her data with multiple service providers (SPs). The fingerprint  of a specific SP is obtained using a cryptographic hash function, whose input is the concatenation of the database owner's secret key and the SP's public series number. For fingerprint insertion, the vanilla scheme  pseudorandomly selects one bit position of one attribute of some data records in the database and replaces those bits with the results obtained from the exclusive or (XOR) between mask bits and fingerprint bits, both of which are also determined pseudorandomly.  
For fingerprint extraction, the scheme locates the exact positions of the potentially changed bits,   calculates the fingerprint bits by XORing those bits with the exact mask bits, and finally recovers each bit in the  fingerprint bit-string via majority voting, since each fingerprint bit can be  used to mark many different positions.
% \footnote{Please refer to Figure 1 on page 36 and Figure 2 on page 37 in \cite{li2005fingerprinting} for the pseudocodes of fingerprint insertion and extraction of the considered vanilla scheme.} 
To preserve the utility of the fingerprinted database, we will let the vanilla scheme only change the least significant bit (LSB) of selected database entries. {\color{black}For completeness,   we show the steps to insert fingerprint into a database, and the steps to extract fingerprint from a pirated   database, in Algorithms \ref{algo:vanilla-insert} and \ref{algo:vanilla-extract}, respectively.} In Appendix \ref{sec:utility_LSB},  we will empirically  validate  that only changing the LSB indeed leads to higher utility than altering one of the least $k$ significant bits (L$k$SB) of selected entries. 




\begin{algorithm}
\small
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{The original relational database $\mathbf{R}$, fingerprinting ratio $\gamma$, database owner's secret key $\mathcal{K}$, pseudorandom number sequence generator $\mathcal{U}$, and the SP's series number $n$ (which can be public).}
\Output{The vanilla fingerprinted relational database $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\emptyset,\emptyset \Big)$.}

Generate the fingerprint bit string of SP $n$, i.e., $f_{\mathrm{SP}_n} = Hash(\mathcal{K}|n)$;

\ForAll{data record $\boldsymbol{r}_i\in\mathbf{R}$}{
\If{$\mathcal{U}_1(\mathcal{K}|\boldsymbol{r}_i.\mathrm{primary\ key})\ \mathrm{mod}\ \gamma = 0$}{
\CommentSty{//fingerprint this data record}

$\mathrm{attribute\_index}\ p = \mathcal{U}_2(\mathcal{K}|\boldsymbol{r}_i.\mathrm{primary\ key})\ \mathrm{mod}\ |\mathcal{F}|$.
\CommentSty{//fingerprint this attribute ($|\mathcal{F}|$ is the cardinality of the attributes set)}


Set $\mathrm{mask\_bit}\ x = 0$, if $\mathcal{U}_3(\mathcal{K}|\boldsymbol{r}_i.\mathrm{primary\ key})$ is even; otherwise set $x=1$.

$\mathrm{fingerprint\_index}\ l=\mathcal{U}_4(\mathcal{K}|\boldsymbol{r}_i.\mathrm{primary\ key})\ \mathrm{mod}\ L$. \CommentSty{//$L$ is the length of the fingerprint bit-string}

$\mathrm{fingerprint\_bit}\ f = f_{\mathrm{SP}_n}(l)$. 


% \CommentSty{//select fingerprint bit position $l$}

$\mathrm{mark\_bit}\ m = x\oplus f$.

 Set the LSB of $\boldsymbol{r}_i.p$ to $m$. %\CommentSty{//$\boldsymbol{r}_i.p$ is the $p$th attribute of the $i$th row in $\mathbf{R}$}

} 


}


 
 Return $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\emptyset,\emptyset \Big)$.

		\caption{Fingerprint insertion phase of the vanilla fingerprinting scheme \cite{li2005fingerprinting}}
\label{algo:vanilla-insert}
\end{algorithm}


\begin{algorithm}
\small
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{The leaked relational database $\overline{\mathbf{R}}$, fingerprinting ratio $\gamma$, database owner's secret key $\mathcal{K}$, pseudorandom number sequence generator $\mathcal{U}$, and a fingerprint template $(?,?,\cdots,?)$, where $?$ represents unknown value.}
\Output{The extracted fingerprint from the leaked database.}

\ForAll{$l\in[1,L]$}{

$count[l][0] = count[l][1] = 0$. \CommentSty{//$count[l][0]$ and  $count[l][1]$ are number of votes for $f(l)$ to be 0 or 1, respectively.}

}

% Generate the fingerprint bit string of SP $n$, i.e., $f_{\mathrm{SP}_n} = Hash(\mathcal{K}|n)$;

\CommentSty{//scan all data records and obtain the counts for each fingerprint bit}

\ForAll{data record $\boldsymbol{r}_i\in\mathbf{R}$}{
\If{$\mathcal{U}_1(\mathcal{K}|\boldsymbol{r}_i.\mathrm{primary\ key})\ \mathrm{mod}\ \gamma = 0$}{ 

$\mathrm{attribute\_index}\ p = \mathcal{U}_2(\mathcal{K}|\boldsymbol{r}_i.\mathrm{primary\ key})\ \mathrm{mod}\ |\mathcal{F}|$.


Set $\mathrm{mark\_bit}\ m$ as the LSB of $\boldsymbol{r}_i.p$.

Set $\mathrm{mask\_bit}\ x = 0$, if $\mathcal{U}_3(\mathcal{K}|\boldsymbol{r}_i.\mathrm{primary\ key})$ is even; otherwise set $x=1$.

$\mathrm{fingerprint\_bit}\ f = m\oplus x$.

$\mathrm{fingerprint\_index}\ l=\mathcal{U}_4(\mathcal{K}|\boldsymbol{r}_i.\mathrm{primary\ key})\ \mathrm{mod}\ L$.

$count[l][f] = count[l][f]+1$.

% \CommentSty{//select fingerprint bit position $l$}



% Set the LSB of $\boldsymbol{r}_i.p$ to $m$.




} 


}

\CommentSty{//recover the fingerprint bit string}

\ForAll{$l\in[1,L]$}{
\If{count[l][0] = count[l][1]}{return none suspected}

$f(l)=0$ if $count[l][0] > count[l][1] = 0$.

$f(l)=1$ if $count[l][0] < count[l][1] = 0$.



}
 
 Return the extracted fingerprint bit string $f$.

		\caption{Fingerprint extraction phase of the vanilla fingerprinting scheme \cite{li2005fingerprinting}}
\label{algo:vanilla-extract}
\end{algorithm}


In practice, one can choose any database fingerprinting scheme as the vanilla scheme, because our proposed mitigation techniques are independent of the adopted vanilla scheme, and they can be used as post-processing steps on top of any existing database fingerprinting schemes. 
The reason we choose the aforementioned  vanilla scheme  is because
% (i) it is a key-based scheme, which uses secret key in each step of the fingerprint insertion and detection, (ii) it does not require storing all the SP-fingerprint pairs in another database for detection purpose, (iii) it processes each data record independently, 
(i) it is shown to have high robustness, e.g., the probability of detecting no fingerprint as a result of random bit flipping attack (a common attack against fingerprinting schemes, as will be discussed in Section~\ref{sec:threat_models}) is upper bounded by ${(|SP|-1)}/{2^L}$, where $|SP|$ is the number of SPs who have received the fingerprinted copies and $L$ is the length of the fingerprint bit-string, (ii) it is shown to be robust even if some fingerprinted entries are identified by a malicious SP, because it applies majority voting on all the fingerprinted entries to extract the fingerprint bit-string, 
and (iii) it can easily be extended to incorporate Boneh-Shaw code \cite{boneh1998collusion} to defend against collusion attacks.  {\color{black}Our developed  robust fingerprinting scheme inherits all the properties of the vanilla  scheme because (i) it uses the  vanilla scheme as the building block and (ii) it does not alter the entries that have already been changed by the vanilla scheme (due to fingerprinting insertion).}



==> sections/proposed_work.tex <==
\section{System and Threat Models}
\label{sec:system-threat}

%\ea{who are the players: database owner (collector) and other parties that receive a (fingerprinted) copy of the database. Provide the notations we use here (preferably have a figure showing the interaction along with the symbols)}

%\ea{Also introduce (with symbols) the utility definition for the database owner and the attacker (along with the considered utility metrics)}

%\ea{who is the attacker: formalize the considered attacks here one by one. For the attacker, define success metrics (confusing the detection algorithm). For the detection algorithm, introduce the ``robustness'' definition. Discuss about the collusion attack, but say we do not consider this attack in this work}

%\hl{in the following: we first show the vulnerability of existing fingerprinting schemes for databases. We should discus why we selected the considered fingerprinting mechanism to show this vulnerability. Then, we propose a new, robust fingerprinting scheme that is robust against the identified vulnerability (and provides high utility at the same time)}

%In this section, 
%\hl{EA: not sure about the number of variable arguments in $\widetilde{\mathbf{R}}(A,B,C,\cdots)$. Can we set it to 3 and use it only for the fingerprinting side? Then, can we use another convention for the attacker, which will have 2 input arguments? You can concatenate those two when you want to show the defense and attack together}


%\hl{EA: lets not use "defense operations". maybe "mitigation techniques"?}





First, we introduce the  nomenclature for different databases obtained by applying various techniques. We denote the database owner's  (i.e., Alice) original database as $\mathbf{R}$, a fingerprinted database shared by her as $\widetilde{\mathbf{R}}$, and the pirated database leaked by a malicious SP as $\overline{\mathbf{R}}$,  respectively. 
Both $\widetilde{\mathbf{R}}$ and $\overline{\mathbf{R}}$ are represented using 3 input parameters showing the techniques that are adopted to generate them.
3 input parameters for $\widetilde{\mathbf{R}}(\alpha,\beta,\eta)$ represent which processes have been applied to the database during fingerprinting, where (i) $\alpha$ represents the vanilla fingerprinting, (ii) $\beta$ represents the proposed mitigation technique against the row-wise correlation attack, and (iii) $\eta$ represents the proposed mitigation technique against the column-wise correlation attack. On the other hand, 3 input parameters for $\overline{\mathbf{R}}(\alpha,\beta,\eta)$ represent which attacks have been conducted by the malicious SP on the fingerprinted database, where (i) $\alpha$ represents the random bit flipping attack, (ii) $\beta$ represents the row-wise correlation attack, and (iii) $\eta$ represents the column-wise correlation attack. We provide the details of these attacks and mitigation techniques in Sections \ref{sec:corr_attacks} and \ref{sec:robust_fp}, respectively. We will also use $\widetilde{\mathbf{R}}$ (or $\overline{\mathbf{R}}$) when referring  to a generic fingerprinted (or pirated) database when its input parameters are clear from the context. 


% \hl{EY: I think such parameters should be introduced later. Dfs should be introduced in Section 6 and Atk in the next subsection (threat model). Here, we mention mitigation techniques without defining system and threat model. Dfs-row and Dfs-col do not make sense before defining row-wise and column-wise attacks. Also, FP parameter can be omitted.} 
We summarize the frequently used notations in  Table~\ref{main_notations}. For instance, $\widetilde{\mathbf{R}}\big(\mathrm{FP},\mathrm{Dfs_{row}(\mathcal{S}')},\mathrm{Dfs_{col}(\mathcal{J}')}\big)$ represents a fingerprinted database that is generated by applying the vanilla fingerprinting scheme ($\mathrm{FP}$) on the original database $\mathbf{R}$ followed by two proposed mitigation techniques $\mathrm{Dfs_{row}(\mathcal{S}')}$ and $\mathrm{Dfs_{col}(\mathcal{J}')}$ to alleviate the potential correlation attacks (as will be discussed in Sections~\ref{sec:col_defense} and~\ref{sec:row-defense}).  
Here, $\mathcal{S}'$ (or $\mathcal{J}'$) is the database owner's prior knowledge on the row-wise (or column-wise) correlations in the database. 
Similarly, $\overline{\mathbf{R}}\big(\emptyset,\mathrm{Atk_{row}(\mathcal{S})},\mathrm{Atk_{col}}(\mathcal{J})\big)$ represents a pirated database that is generated by a malicious SP by first launching the row-wise correlation attack $\mathrm{Atk_{row}}(\mathcal{S})$, and then the column-wise correlation attack $\mathrm{Atk_{col}}(\mathcal{J})$ (as will be discussed in Section~\ref{sec:col-wise-attack} and \ref{sec:row-wise-atack}, and $\emptyset$ means random bit flipping attack is not applied).  
Here, $\mathcal{S}$ (or $\mathcal{J}$) is the malicious SP's prior knowledge on the row-wise (or column-wise) correlations of the database.   
In general, $\mathcal{S}'\neq\mathcal{S}$ and $\mathcal{J}'\neq\mathcal{J}$, which is referred to as the prior knowledge asymmetry between the database owner and the malicious SP. To the advantage of the malicious SP, we assume that the malicious SP can have access to the correlation models that are directly calculated from the database, i.e., its prior knowledge is as accurate as that of the database owner. 
In the future work, we will also   investigate the scenario where the database owner even has less accurate prior knowledge compared with the malicious SPs.
%   In what follows, we discuss the system model, threat model, and utility metrics.


\begin{table*}[htb]
\begin{center}
 \begin{tabular}{c | c  } 
 \hline
 \hline
%  Notions & Descriptions \\ 
%   \hline
  $\mathbf{R}$ & the  original database owned by the database owner (Alice)\\
   \hline
   $\widetilde{\mathbf{R}}$ & a generic fingerprinted database shared by the database owner\\
   \hline
   $\overline{\mathbf{R}}$ & a generic pirated database generated by the malicious SP\\
   \hline
%   $\mathbf{R}_\kappa$ & a random database obtained by keeping $\kappa$ percentage of data records in $\mathbf{R}$ randomly \\
        % \hline
  \multirow{3}{*}{$\widetilde{\mathbf{R}}(\alpha,\beta,\eta)$} & the fingerprinted database obtained by applying   (i) $\alpha$, the vanilla fingerprinting scheme,  \\
  & (ii) $\beta$, the mitigation technique against the row-wise correlation attack,  \\
   & and (iii) $\eta$, the mitigation technique against the column-wise correlation attack  in sequence\\
   \hline
   \multirow{2}{*}{$\overline{\mathbf{R}}(\alpha,\beta,\eta)$} & the pirated database generated by the malicious SP by applying (i) the random bit flipping attack $\alpha$, \\
   & (ii) the row-wise correlation attack $\beta$,  and (iii) the column-wise correlation attack $\eta$ in sequence\\
   \hline
  $\mathcal{S}'$ and $\mathcal{J}'$ & database owner's prior knowledge on the row-wise correlations and column-wise correlations\\
  \hline
    $\mathcal{S}$ and $\mathcal{J}$ & the malicious SP's prior knowledge on the row-wise correlations and column-wise correlations\\
  \hline
    $\widetilde{\mathcal{S}}$ and $\widetilde{\mathcal{J}}$ & the empirical row-wise and column-wise correlations obtained from a generic  fingerprinted database $\widetilde{\mathbf{R}}$\\
% \hline
%   $\mathrm{Atk_{rnd}}$ & the random bit flipping attack\\
%   \hline  $\mathrm{Atk_{row}}(\mathcal{S})$ & the row-wise correlation attack launched by the malicious SP by using prior knowledge $\mathcal{S}$ \\
    \hline
 $\mathrm{Atk_{col}}(\mathcal{J})$ & the column-wise correlation attack launched by the malicious SP by using prior knowledge $\mathcal{J}$ \\ 
   \hline
  $\mathrm{Dfs_{row}}(\mathcal{S}')$ & the mitigation technique using prior knowledge $\mathcal{S}'$  to alleviate row-wise correlation attack \\
    \hline
  $\mathrm{Dfs_{col}}(\mathcal{J}')$ & the mitigation technique using prior knowledge $\mathcal{J}'$  to alleviate column-wise correlation attack \\
 \hline
 \hline
\end{tabular}
% \end{minipage}}
\caption{Frequently used notations in the paper.}
% \hl{EA: we should further simplify this table. Lets talk about this (you can check my representation of the parameters in the text)}} 
\label{main_notations}
\end{center}
\end{table*}




% \begin{figure*}
%   \begin{center}
%   \begin{tabular}{ccc}
%   \hspace{-7mm}
%      \includegraphics[width= .66\columnwidth]{figures/fp_general_system.jpg}
% 		&
% 		\hspace{-8mm}
% 		     \includegraphics[width= 1.66\columnwidth]{figures/common_attacks.jpg}
%      \\
%     {\small  (a) Fingerprinting system.}  &
%     {\small  (b) Attacks considered in this paper.}\\
%         \end{tabular}
%       \end{center}
%   \caption{\label{fig:system_and_attacks} (a) The vanilla fingerprinting system, where Alice adds a unique fingerprint in each shared copy of her database. She is able to identify the malicious SP who pirates and redistributes her database {\color{black}as long as the data entries are not significantly modified (e.g., when less than 80\% of the entries are changed or removed)}. (b) Representative attacks considered in this paper. (i) If Alice inserts fingerprinting using the vanilla scheme, and the malicious $\mathrm{SP}_i$ conducts random bit flipping attack, i.e., $\mathrm{Atk_{rnd}}$, on its received copy, i.e.,   $\widetilde{\mathbf{R}}_{\mathrm{SP}_i}(\mathrm{FP},\emptyset,\emptyset)$ and redistributes the data. Then, with high probability, Alice can correctly accuse it for data leakage. (ii) If the malicious $\mathrm{SP}_i$ conducts any correlation attack, e.g., the column-wise correlation attack ($\mathrm{Atk_{col}}(\mathcal{J})$), the row-wise correlation attack ($\mathrm{Atk_{row}}(\mathcal{S})$), or the combination of them, on the vanilla fingerprinted database. Then, with high probability, Alice cannot identify it as the traitor, and she will accuse other innocent SPs. (iii)  If Alice applies the mitigation techniques, i.e., the column-wise correlation defense ($\mathrm{Dfs_{col}}(\mathcal{J}')$) and the row-wise correlation defense ($\mathrm{Dfs_{row}}(\mathcal{S}')$), after the vanilla fingerprinting scheme, and shares $\widetilde{\mathbf{R}}(\mathrm{FP},\mathrm{Dfs_{row}}(\mathcal{S}'),\mathrm{Dfs_{col}}(\mathcal{J}'))$ with $\mathrm{SP}_i$. Then, with high probability, she can correctly identify $\mathrm{SP}_i$ as the traitor even if it conducts any of the correlation attack on its received copy.}
% \end{figure*}

\subsection{System Model}
\label{system_model}

% \hl{EA: $|\mathcal{F}|=L$? then why do you use two different letters? also $r$ should have an index right?} 



% \hl{EA: instead of $fp$, can you use only $f$ or $p$? Also should be have an index for $\widetilde{\mathbf{R}}$, showing which SP received it?} 




We present the vanilla   fingerprint system model  in Figure \ref{fig:fp_general_system}. Specifically, we consider the database owner (Alice) with a  {categorical} relational database   $\mathbf{R}$, which includes the data records of $M$ individuals.  We denote the set of attributes of the individuals as $\mathcal{F}$ and the $i$th row (data record) in $\mathbf{R}$ as $\boldsymbol{r}_i$. 
% {\color{blue}Besides, we use $\mathbf{R}.(i,p)$ to represent the query of attribute $p$ ($p\in\mathcal{F}$) of the $i$th record, and let $\mathbf{R}.p$ represent querying attribute $p$ of all the records.} 
Alice shares her data with multiple service providers (SPs) 
% , such as Amazon Web Services and Apple Cloud, 
to  receive specific services from them. To prevent unauthorized redistribution of her database by a malicious SP, Alice includes a unique fingerprint in each copy of her database when sharing it with a SP. The fingerprint bit-string associated to SP $i$ ($\mathrm{SP}_i$) is denoted as $f_{\mathrm{SP}_i}$, and the vanilla fingerprinted dataset received by $\mathrm{SP}_i$ is represented as $\widetilde{\mathbf{R}}_{\mathrm{SP}_i}(\mathrm{FP},\emptyset,\emptyset)$. 
Both $f_{\mathrm{SP}_i}$ and $\widetilde{\mathbf{R}}_{\mathrm{SP}_i}(\mathrm{FP},\emptyset,\emptyset)$ are obtained  using the vanilla fingerprint scheme discussed in Section \ref{sec:vanilla}, which changes entries of $\mathbf{R}$ at different positions (indicated by the yellow dots in Figure \ref{fig:fp_general_system}.   
If a malicious SP (e.g., $\mathrm{SP}_i$)   pirates and  redistributes Alice's database, she is able to identify $\mathrm{SP}_i$ as the traitor by extracting its fingerprint in $\widetilde{\mathbf{R}}_{\mathrm{SP}_i}(\mathrm{FP},\emptyset,\emptyset)$ {\color{black}as long as the data entries are not significantly modified (e.g., when less than 80\% entries are changed or removed)}. 

% \hl{EA: in general, use "her" for the data owner (Alice) and use "it/its" for the SP. Currently there are also him/his for the SP}

\begin{figure}[htb]
  \begin{center}
     \includegraphics[width= 0.7\columnwidth]{figures/fp_general_system.jpg}
      \end{center}
  \caption{\label{fig:fp_general_system}  The vanilla fingerprinting system, where Alice adds a unique fingerprint in each shared copy of her database. She is able to identify the malicious SP who pirates and redistributes her database {\color{black}as long as the data entries are not significantly modified (e.g., when less than 80\% of the entries are changed or removed)}.}
\end{figure}





\begin{figure*}[htb]
  \begin{center}
     \includegraphics[width= 1.65\columnwidth]{figures/common_attacks.jpg}
      \end{center}
  \caption{\label{fig:attacks}   (i) If Alice inserts fingerprinting using the vanilla scheme, and the malicious $\mathrm{SP}_i$ conducts random bit flipping attack, i.e., $\mathrm{Atk_{rnd}}$, on its received copy, i.e.,   $\widetilde{\mathbf{R}}_{\mathrm{SP}_i}(\mathrm{FP},\emptyset,\emptyset)$ and redistributes the data. Then, with high probability, Alice can correctly accuse it for data leakage. (ii) If the malicious $\mathrm{SP}_i$ conducts any correlation attack, e.g., the column-wise correlation attack ($\mathrm{Atk_{col}}(\mathcal{J})$), the row-wise correlation attack ($\mathrm{Atk_{row}}(\mathcal{S})$), or the combination of them, on the vanilla fingerprinted database. Then, with high probability, Alice cannot identify it as the traitor, and she will accuse other innocent SPs. (iii)  If Alice applies the mitigation techniques, i.e., the column-wise correlation defense ($\mathrm{Dfs_{col}}(\mathcal{J}')$) and the row-wise correlation defense ($\mathrm{Dfs_{row}}(\mathcal{S}')$), after the vanilla fingerprinting scheme, and shares $\widetilde{\mathbf{R}}(\mathrm{FP},\mathrm{Dfs_{row}}(\mathcal{S}'),\mathrm{Dfs_{col}}(\mathcal{J}'))$ with $\mathrm{SP}_i$. Then, with high probability, she can correctly identify $\mathrm{SP}_i$ as the traitor even if it conducts any of the correlation attack on its received copy.}
\end{figure*}








\subsection{Threat Model}
\label{sec:threat_models}
Fingerprinted database is subject to various attacks summarized in the following sections. In Figure \ref{fig:attacks}, we show some representative ones that are studied in this paper. 
Note that in all considered attacks, a malicious SP can change/modify most of the entries in $\widetilde{\mathbf{R}}$ to distort the fingerprint (and to avoid being accused). However, such a pirated database will have significantly poor utility (as will be introduced in Section \ref{sec:utility_metrics}).  {\color{black}As discussed in Section \ref{sec:vanilla}, we let the vanilla fingerprint scheme only change the LSBs of data entries to preserve data utility. Thus, all considered attacks also change the LSBs of the selected entries in $\widetilde{\mathbf{R}}$ to distort the fingerprint.}

% Thus, in this work, to preserve the database utility, we  assume that some of the  attacks just change the LSB of the selected entries in $\widetilde{\mathbf{R}}$ to distort the fingerprint. As we show in Appendix \ref{sec:utility_LSB}, changing the LSB of the database entries results in the least utility loss.


\subsubsection{Random Bit Flipping Attack} In this attack, to pirate a database, a malicious SP   selects  random entries in $\widetilde{\mathbf{R}}$ and flips their LSBs \cite{agrawal2003watermarking}. The flipped entries are still in the domain of the corresponding attributes. 
The considered vanilla fingerprint scheme is robust against this attack \cite{li2005fingerprinting} as shown in Figure~\ref{fig:attacks}(i),   Alice shares fingerprinted copies of her database by only applying  $\mathrm{FP}$. If a malicious SP ($\mathrm{SP}_i$) tries to distort the fingerprint in $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$ using the random bit flipping attack (i.e., $\mathrm{Atk_{rnd}}$), and then   redistributes it, Alice can still detect $\mathrm{SP}_i$'s fingerprint in the pirated  copy with a high probability, 
% \hl{EA: should we say "with a high probability" here? if the SP over-distors the database, Alice cannot detect, right?}   
and correctly accuse $\mathrm{SP}_i$ of data leakage.
% In fact, to distort more than half of the fingerprint bits, $\mathrm{Atk_{rnd}}$ needs to change more than $83\%$ of the database entries (as we will show in Section \ref{sec: int_attack_census}), which compromise the database utilities significantly. 


\subsubsection{Subset and Superset Attacks}
In subset attack, a malicious SP generates a pirated copy of $\widetilde{\mathbf{R}}$ by randomly selecting  data records from it.   Superset attack is the dual attack of subset attack. In this attack, the malicious SP mixes $\widetilde{\mathbf{R}}$ with other databases to create a pirated  one. These two attacks are considered to be  weak attacks. For example, for subset attack, to compromise just one specific  bit in the inserted  fingerprint bit-string,  the malicious SP must exclude all records that are marked by that  bit~\cite{li2005fingerprinting}.














\subsubsection{Correlation Attacks}
In correlation attacks, a malicious SP utilizes the inherent correlations in the data to more accurately identify the fingerprinted entries, and hence distort the fingerprint. 
Since the subset and superset attack are not as powerful as the bit flipping attack \cite{yilmaz2020collusion}, we consider developing the correlation attacks based on the random bit flipping attack. In the following, we provide the high level descriptions of two main correlation attacks (details of these attacks are in Section \ref{sec:corr_attacks}).

%\hl{EA: do we still call this pairwise only? or can we just say correlations between columns?} 


%\hlgreen{tj: need to discuss, the algorithm is described in terms of pairwise, but also mentioned higher order correlations later.}


In column-wise correlation attack, i.e., $\mathrm{Atk_{col}}(\mathcal{J})$, we assume that the malicious SP has prior knowledge about the correlations among each pair of attributes  (or columns in the database) characterized by the set of joint probability distributions $\mathcal{J}$. Once receiving the fingerprinted  database $\widetilde{\mathbf{R}}$, the malicious SP first calculates a new set of joint probability distributions based on  $\widetilde{\mathbf{R}}$.  %(denoted as  $\mathcal{J}(\widetilde{\mathbf{R}})$). 
Then, it compares %$\mathcal{J}(\widetilde{\mathbf{R}})$ 
the new joint distributions with its prior knowledge $\mathcal{J}$, and flips the entries in $\widetilde{\mathbf{R}}$ that leads to large discrepancy between them.

% e two sets of correlations. % $\mathcal{J}(\widetilde{\mathbf{R}})$ and $\mathcal{J}$.


% \hl{EA: what does this mean? can we just say it knows the statistical relationship between the records in the database?}

% \hlgreen{tj: needs discussion, we assume the affiliation before and after fp is not changed.}

% \hl{EA: I think you should say what you mean by "affiliation" first"}

In row-wise correlation attack,  i.e., $\mathrm{Atk_{row}}(\mathcal{S})$, we consider that the individuals belong to  different communities (e.g.,  social circles decided by friendship,  or families determined by kinship), and assume that the malicious SP has the prior knowledge $\mathcal{S}$, which contains (i) each individual's membership  to the communities and (ii) the statistical relationships of   pairs of individuals belonging to  the same community.  
Once it receives the fingerprinted  database $\widetilde{\mathbf{R}}$, the malicious SP first calculates a new set of statistical relationships based on $\widetilde{\mathbf{R}}$, then it compares the newly computed  statistical relationships with   $\mathcal{S}$, and changes the entries that leads to large discrepancy between the two sets of statistical relationships.  % $\mathcal{S}(\widetilde{\mathbf{R}},C)$ and $\mathcal{S}$.
% {\color{blue}Note that sometimes the malicious SP can generate  and release synthetic database from  its prior knowledge on column- and row-wise correlations using machine learning models, but it has been empirically show that such database will have relatively large differences to the original data, and has potentially negative effects on
% the utility \cite{hittmeir2019utility}. Thus, }





Figure~\ref{fig:attacks}(ii) shows the scenario, where Alice identifies the source of the data leakage wrong and accuses innocent SPs if she uses the vanilla fingerprinting scheme, whereas, $\mathrm{SP}_i$ conducts more advanced attacks to distort the fingerprint. These attacks include   $\mathrm{Atk_{col}}\big(\mathcal{J}\big)$,   $\mathrm{Atk_{row}}\big(\mathcal{S}\big)$, and the combination of them. Finally, Figure~\ref{fig:attacks}(iii) shows that if Alice uses  the proposed mitigation  techniques (i.e., $\mathrm{Dfs_{row}}(\mathcal{S}')$ and  $\mathrm{Dfs_{col}}(\mathcal{J}')$ (as will be discussed in Section~\ref{sec:robust_fp}) after $\mathrm{FP}$ to improve the robustness of the added fingerprint and shares $\widetilde{\mathbf{R}}\big(\mathrm{FP},   \mathrm{Dfs_{row}}(\mathcal{S}'), \mathrm{Dfs_{col}}(\mathcal{J}')\big)$, % with the SPs,
then, even though $\mathrm{SP}_i$ conducts the identified  correlation attacks, Alice can still identify $\mathrm{SP}_i$ to be responsible for leaking the data with high probability.  



\subsubsection{Collusion Attack}
Fingerprinted databases are also susceptible to collusion attack, where multiple malicious SPs ally together to generate a pirated database from their unique fingerprinted copies. In   cryptography literature, many works have attempted to develop collusion resistant fingerprinting schemes  \cite{boneh1998collusion,boneh1995collusion,yacobi2001improved,pfitzmann1997asymmetric}.  Our proposed mitigation techniques can also be used with a collusion-resistant vanilla fingerprinting scheme \cite{boneh1998collusion} to   provide some level of robustness against colluding SP.  In this work, we   mainly focus on   correlation attacks from a single-handed malicious SP. We will extend our work in the scenario of colluding SPs in future work. 

% and develop corresponding mitigation techniques. 





\subsection{Fingerprint Robustness Metrics}
\label{sec:robustness_metrics}

The primary goal of a malicious SP is to distort the   fingerprint in $\widetilde{\mathbf{R}}$, thus we consider the following fingerprint  robustness metrics about a pirated  database  $\overline{\mathbf{R}}$ generated by launching attacks on $\widetilde{\mathbf{R}}$.
% \begin{itemize}
    
\subsubsection{Number of compromised fingerprint bits}

We formulate the number of compromised fingerprint bits as
    \begin{equation*}
        \mathrm{num_{cmp}} = {\textstyle\sum}_{l = 1}^L \mathbf{1}\{f(l)\neq \overline{f}(l)\},
    \end{equation*}
    where $\mathbf{1}\{\cdot\}$ is the indicator function, $L$ is the length of the fingerprint bit-string, $\overline{f}$ is the extracted  fingerprint bit-string from  $\overline{\mathbf{R}}$, and $f(l)$ (or $\overline{f}(l)$) is the $l$th bit in $f$ (or $\overline{f}$).





\subsubsection{Accusable ranking of a malicious SP}

We quantify the confidence of accusing the correct malicious SP by defining the accusable ranking metric (denoted as $r$) as follows: 
\begin{gather*}
r = 
\begin{cases}
&\mathrm{``uniquely\ accusable"},  \textit{if}\  m_0 >  \sum_{l=1}^L\mathbf{1}\Big\{f_{\mathrm{SP}_i}(l) = \overline{f}(l)\Big\},  \forall \mathrm{SP}_i \in \mathcal{T}  \\
&\mathrm{``top}\ t\ \mathrm{accusable"} , \textit{otherwise}
\end{cases},
\end{gather*}
where   $m_0 = \sum_{l=1}^L\mathbf{1}\{f_{\mathrm{SP_{malicious}}}(l) = \overline{f}(l)\}$ is the number of bit matches between the malicious SP's fingerprint and the extracted fingerprint from the pirated database, and $\mathcal{T}$ is the set of all innocent SPs. Specifically, if the malicious SP has the most bit matches with the extracted fingerprint,   Alice will uniquely accuse it. Otherwise, we compute $t=\frac{\sum_{\mathrm{SP}_i \in \mathcal{T}} \mathbf{1}\Big\{\Big(\sum_{l=1}^L\mathbf{1}\Big\{f_{\mathrm{SP}_i}(l) = \overline{f}(l)\Big\}\Big) \geq m_0\Big\}} {|\mathcal{T}|}\times 100\%$,
which is  the fraction  of innocent SPs having more bit matches with the extracted fingerprint than the malicious SP. For example, if $t = 80\%$, then the malicious SP is only top 80\% accusable, which suggests that Alice will accuse other innocent SPs with high probability. In contrast, if $t = 1\%$, then the malicious SP's accusable ranking increases and makes it among the top 1\% accusable SPs, and Alice will accuse other innocent SPs with low probability. Essentially, a high accusable rank $r$ corresponds to either (i) a ``low $t$" or (ii) the uniquely accusable case. 
{\color{black}As we will show in Section \ref{sec:eva}, for a malicious SP to avoid being accused (i.e., have low accusable rank, or high $t$ value),  it needs to distort more than half of the fingerprint bits. As we will also show via evaluations, the malicious SP can easily achieve this goal if it applies the identified  correlation attacks. Whereas, if it applies the random bit flipping attack, it becomes ``uniquely accusable'' with high probability unless it overdistort the fingerprinted database.}



% In Section~\ref{sec: int_attack_census}, we  will show that unless it distorts more than half of the fingerprint bits, a malicious SP will have a high accusable rank (with a low $t$ value), but using the identified  correlation attacks, the malicious SP can easily increase the value of $t$ to achieve a low accusable rank. Whereas,   random bit flipping attack   leads to the ``uniquely accusable'' case with high probability.  {\color{blue}Furthermore, in Section \ref{sec:eva}, we will show that the SPs that are identified  as ``uniquely accusable'' are all real traitors who release the database.}

{\color{black}
According to the vanilla scheme~\cite{li2005fingerprinting}, the probability of extracting a valid fingerprint from a database that does not belong to Alice (i.e., misdiagnosis false hit) is upper bounded by $|\mathrm{SP}|/2^L$, and the probability of extracting an incorrect but valid fingerprint from the fingerprinted database (i.e., misattribution false hit) is upper bounded by $(|\mathrm{SP}|-1)/2^L$. Since these are all negligible probabilities, we do not consider the case in which Alice does not accuse any SP when a copy of her database is leaked in the experiments.
}




\subsection{Utility Metrics}
\label{sec:utility_metrics}

% \hl{EA: also need to mention the attacker's utility (and highlight that the attacker can succeed easily by over-distorting. But, a rational attacker does not want to over-distort  due to its utility requirement)}

Fingerprinting naturally changes the content of the database, and hence degrades its utility. 
We quantify the utility of a fingerprinted database using the following metrics. 
% \begin{itemize}

\subsubsection{Accuracy of $\widetilde{\mathbf{R}}$} 

We quantify the accuracy of $\widetilde{\mathbf{R}}$ as  
\begin{equation*}
      Acc(\widetilde{\mathbf{R}}) = 1-  {\widetilde{\mathbf{R}}\oplus \mathbf{R}}/{M*L},
  \end{equation*}
  where $\oplus$ is the symmetric difference operator that counts   the number of different entries in the fingerprinted and the original databases. $Acc(\widetilde{\mathbf{R}})$ measures the percentage of matched entries between the    fingerprinted and the original databases. % (higher $Acc(\widetilde{\mathbf{R}})$ means higher utility for $\widetilde{\mathbf{R}}$). 
  
\subsubsection{Preservation of column-wise correlations}

We quantify the preservation of column-wise correlations in the database as
  \begin{gather*}
    \mathrm{P_{col}}(\widetilde{\mathbf{R}}) = 1 - \frac{\sum_{p,q\in \mathcal{F},p\neq q}\sum_{a\in p, b\in q} \mathbf{1}\big\{ \big| \widetilde{J_{p,q}}(a,b)-J_{p,q}(a,b)  \big| \geq\tau_{\mathrm{col}} \big\}}{\sum_{p,q\in \mathcal{F},p\neq q} k_pk_q},
\end{gather*}
  where $p$ and $q$ are two attributes in the attribute set $\mathcal{F}$, $k_p$ (or $k_q$) stands for the number of unique instances of attribute $p$ (or $q$), and $\widetilde{J_{p,q}}(a,b)$ (or $J_{p,q}(a,b)$) is the joint probability that attribute $p$ takes value $a$ and attribute $q$ takes value $b$ in $\widetilde{\mathbf{R}}$ (or $\mathbf{R}$). %, and $\mathbf{1}\{\cdot\}$ is the indicator function. 
    $\mathrm{P_{col}}$ calculates the fraction of instances of $\big| \widetilde{J_{p,q}}(a,b)-J_{p,q}(a,b)  \big| $ that do not exceed a predetermined threshold $\tau_{\mathrm{col}}$ before and after fingerprinting $\mathbf{R}$. 
  
\subsubsection{Preservation of row-wise correlations}

We quantify the preservation of row-wise correlations in the database as
    \begin{gather*}
        \mathrm{P_{row}}(\widetilde{\mathbf{R}}) = 1 - \frac{\sum_{c=1}^C\sum_{i,j\in\mathrm{comm}_c,i\neq j}\mathbf{1}\big\{\big|\widetilde{s_{i,j}}^{\mathrm{comm}_c}-s_{i,j}^{\mathrm{comm}_c}\big| \geq \tau_{\mathrm{row}}\big\}}{\sum_{c=1}^C n_c(n_c-1)},
    \end{gather*}
where $\mathrm{comm}_c$ represents the set of all individuals in a community $c$,   $\widetilde{s_{i,j}}^{\mathrm{comm}_c}$ (or $s_{i,j}^{\mathrm{comm}_c}$) is the statistical relationship between individual $i$ and $j$ belonging to $\mathrm{comm}_c$ in $\widetilde{\mathbf{R}}$ (or $\mathbf{R}$),   $n_c$ is the number of individuals in $\mathrm{comm}_c$, and $C$ is the number of communities. In essence, $\mathrm{P_{row}}(\widetilde{\mathbf{R}})$ evaluates the fraction of    statistical relationship that has absolute  difference   less than $\tau_{\mathrm{row}}$ in the entire population before and after fingerprinting. 

\subsubsection{Preservation of empirical covariance matrix}

We quantify the preservation of  empirical covariance matrix of the database as
  \begin{equation*}
      \mathrm{P_{cov}} = 1-{||\mathrm{cov}(\widetilde{\mathbf{R}})-\mathrm{cov}(\mathbf{R})||_F}/ {||\mathrm{cov}(\mathbf{R})||_F},
  \end{equation*}
  where $\mathrm{cov}(\mathbf{R}) = \sum_{i=1}^M \boldsymbol{r}_i^T\boldsymbol{r}_i/M$ is the empirical covariance matrix of data records in $\mathbf{R}$. $\mathrm{P_{cov}}$ evaluates the similarity between the covariance matrices of the database before and after fingerprinting. We consider this metric because the fingerprinted database may also be used in data analysis tasks, and  empirical covariance matrix is frequently utilized  to   establish  predictive models, e.g., regression and probability fitting \cite{jolliffe2002springer,browne1992alternative}. Besides,   multivariate data analysis often involves the investigation of  inter-relationships among data records which requires an accurate covariance matrix estimation. 
%   \hl{EY: Can we add preservation of statistics (e.g., mean of columns etc.) or query results?}
%   \hlgreen{TJ: how about just using the empirical covariance matrix, i.e., $R^TR/M$?} \hl{EA: ok but also try to say why covarience matrix is significant (e.g., examples of how it can be used for database analysis)} 
% \end{itemize}

Note that the utility of the pirated database $\overline{\mathbf{R}}$ generated by the malicious SP can also be quantified using the same metrics, i.e., $Acc(\overline{\mathbf{R}})$, $\mathrm{P_{col}}(\overline{\mathbf{R}})$,    $\mathrm{P_{row}}(\overline{\mathbf{R}})$, and $\mathrm{P_{cov}}(\overline{\mathbf{R}})$. As discussed, a malicious SP can successfully (without being accused) distort the fingerprint easily by over-distorting $\widetilde{\mathbf{R}}$, however, to preserve the data utility, a rational malicious SP will not over-distort a database.

% to preserve the utility of the original database (we show how the utility of the malicious SP degrades as a result of the attacks in Section \ref{sec:corr_attacks}). 


{\color{black}

In addition to the general utility metrics defined above, we will also consider specific statistical utilities, e.g., portion of individuals that have a particular education degree or higher, and the standard deviation of individuals' age distribution. It is noteworthy that  if the general utility metrics are high, it  implicitly suggests high utility for the specific statistical (or other application  related) utilities.}




\section{Identified Correlation Attacks}
\label{sec:corr_attacks}

% \hl{EA: reconsider the title}
%\ea{Lets have the highlevel descriptions of these attacks in the threat model}

%\ea{We need the written description of the algorithm as well}



In the correlation attacks, we assume that the malicious SP has access to both column- and row-wise correlations of Alice's database, which contains (i) correlations between all pairs of attributes (columns), (ii) each individual's membership to the communities and (iii) the statistical relationships of pairs of individuals belonging to  the same community. 
% \hl{EA: relationship between the knowledge of affiliations and row-wise correlations are not clear. If the row-wise correlations are high between two people, they are have similar affiliations, right? Do we need to list them separately? Also, is the community and affiliation the same thing? If so, lets stick to one, if not can you mention their difference?} 
Specifically, the column-wise correlations are characterized by the set of joint distributions among pairs %\hl{EA: do we say pairs or do we generalize this? We can also say we say pairs here for simplicity, but we tried more as well} 
of attributes (columns) in the database, i.e., $\mathcal{J} = \{J_{p,q}|p,q\in\mathcal{F},p\neq q\}$. Row-wise correlations, on the other hand, are characterized by the set of statistical relationships between pairs of individuals (rows) in a community. For instance,  $\mathcal{S} = \{s_{ij}^{\mathrm{comm}_c}|i,j\in\mathrm{comm}_c, i\neq j, c\in[1,C]\}$, where $s_{ij}^{\mathrm{comm}_c} = e^{-\mathrm{dist}(\boldsymbol{r}_i,\boldsymbol{r}_j)}$ is the statistical relationship between individuals (data records) $i$ and $j$ in community $\mathrm{comm}_c$ ($\mathrm{dist}(\boldsymbol{r}_i,\boldsymbol{r}_j)$ denotes the Hamming distance between $\boldsymbol{r}_i$ and $\boldsymbol{r}_j$). %, and $C$ is the total number of communities.  
Since the added fingerprint changes some entries in the original  database, which will lead to the change of both joint distributions and statistical relationships, the malicious SP can utilize its auxiliary (publicly available) information about $\mathcal{J}$ and $\mathcal{S}$ to identify the positions of suspicious entries in $\widetilde{\mathbf{R}}$ that are potentially fingerprinted. 




 

\subsection{Column-wise Correlation Attack}
\label{sec:col-wise-attack}

% \hl{EA: lets use "it" for the malicious SP everywhere}

To launch the column-wise correlation attack ($\mathrm{Atk_{col}(\mathcal{J})}$) on  $\widetilde{\mathbf{R}}$, the malicious SP first calculates the empirical joint distributions among pairs of attributes in $\widetilde{\mathbf{R}}$, denoted as $\widetilde{\mathcal{J}}$. 
%\hl{EA: $\widetilde{J_{p,q}}$ and $\widetilde{J_{p,q}}(a,b)$ are not introduced before I think.} 
% \hlgreen{now mentioned in the def of $P_{col}(R)$}
Then, it compares each joint distribution in $\widetilde{\mathcal{J}}$ (i.e., $\widetilde{J_{p,q}}$) with that in $\mathcal{J}$ (i.e., $J_{p,q}$). For instance, if the absolute  difference of joint probabilities when attribute $p$ takes value $a$ and attribute $q$ takes value $b$ (i.e., $\big|J_{p,q}(a,b)-\widetilde{J_{p,q}}(a,b)\big|$) is higher than a threshold $\tau_{\mathrm{col}}^{\mathrm{Atk}}$, then, the malicious SP queries the row indices 
% \hl{EA: are these the row indices only, or the row/column indices?} 
% \hlgreen{TJ: I mean the row indices, we need to distinguish indices and identification keys} 
of the data records in $\widetilde{\mathbf{R}}$ whose attributes $p$ and $q$ take values $a$ and $b$, respectively, and collects the corresponding row indices in a set $\mathcal{I}$, i.e., for the previous example, $\mathcal{I} =  \text{row\ index\ query}\big(\widetilde{\mathbf{R}}.p == a\  \text{and}\ \widetilde{\mathbf{R}}.q == b\big)$  ($\widetilde{\mathbf{R}}.p$ includes   attribute $p$ of all data record in database $\widetilde{\mathbf{R}}$).  
% \hl{EA: you dont say later in the text how this set $\mathcal{I}$ is used to create $\mathcal{P}$ (it is in the algorithm, but we should also connect it to the rest of the discussion in the text as well)}
% \hl{EA: instead of i and j, dont you need to use a and be here?}. 
%We assume that $J_{p,q}(a,b)$ is the malicious SP's prior knowledge on the joint probability of attribute $p$ taking value $a$ and attribute $q$ taking value $b$,  and $\widetilde{J_{p,q}}(a,b)$ is the joint probability of attribute $p$ taking value $a$ and attribute $q$ taking value $b$ in the fingerprinted database $\widetilde{\mathbf{R}}$. 
{\color{black}For each row index $i\in\mathcal{I}$, either position $\{i,p\}$ or $\{i,q\}$ (i.e., the row index and attribute tuple) can be   potentially fingerprinted, because they both affect the joint distribution $\widetilde{J_{p,q}}(a,b)$}. Thus, the malicious SP adds each of {\color{black}these tuples}, i.e.,  $\{i,p\}$ and $\{i,q\}, i\in\mathcal{I}$ into   a suspicious position set denoted as $\mathcal{P}$. % (unless it has been previously included in  $\mathcal{P}$). 
% \hl{EA: as in the above comment, here the connection between sets I and P is missing} 
%\hl{EA: not clear how you use $\mathcal{I}$ in this last step, can you clarify. Also use a different (if possibly one letter) representation for suspicious position set (and also for HSP). We use SP a lot for service providers.}


Since a specific suspicious row index $i$ 
%\hl{EA: as I mentioned before, I think r needs an index (sub or superscript)} 
can be associated with multiple attributes  in  the suspicious position set $\mathcal{P}$, the suspicious  attribute that is most frequently associated with $i$ is considered to be \textbf{highly suspicious}. 
The malicious SP collects these highly suspicious combinations of row index and attribute in a set $\mathcal{H} = \mathcal{H}\cup\{i,\mathrm{mode}(\mathcal{A}_i)\}$, where $\mathcal{A}_i$ includes all the attributes that are paired with row index $i$ in set $\mathcal{P}$, and $\mathrm{mode}(\mathcal{A}_i)$ returns the most frequent attribute in $\mathcal{A}_i$ (if there is a tie,  the malicious SP randomly chooses one). 
% \footnote{If there is a tie between the most frequent suspicious  attributes associated with row index $i$, then, the malicious SP randomly chooses one.} 
Then, the malicious SP launches the column-wise correlation attack by flipping the LSB of entries in $\widetilde{\mathbf{R}}$ whose positions are in $\mathcal{H}$, i.e., $\widetilde{\mathbf{R}}.(i,p), \forall \{i,p\}\in\mathcal{H}$  {\color{black}($\widetilde{\mathbf{R}}.(i,p)$ represents the value of attribute $p$ for the $i$th data record in   $\widetilde{\mathbf{R}}$)}.


In practice, the malicious SP can launch multiple rounds of $\mathrm{Atk_{col}(\mathcal{J})}$ by iteratively comparing the new joint distributions obtained from the attacked fingerprinted database in the previous round with its prior knowledge $\mathcal{J}$. 
In each round,  a new $\mathcal{H}$ is constructed, but the malicious SP does not flip the highly suspicious positions that have already been flipped in previous rounds. This can be achieved by maintaining and updating an accumulative highly suspicious position set $\mathcal{Z}$. We summarize the steps of conducting $t$ rounds of $\mathrm{Atk_{col}(\mathcal{J})}$ in
Algorithm \ref{Algo:col-wise-attack}. % in Appendix~\ref{sec:supp_algos_col-wise-attack}.

\begin{algorithm}
\small
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Fingerprinted   database $\widetilde{\mathbf{R}}$, malicious SP's prior knowledge on the pairwise joint distributions among attributes, $\mathcal{J}$, and attack rounds $t$.}
\Output{column-wise correlation attacked   DB  $\overline{\mathbf{R}}\Big(\emptyset,\emptyset,\mathrm{Atk_{col}}(\mathcal{J})\Big)$.}

Initialize $cnt = 1$;

Initialize  $\mathcal{Z} = \emptyset$;

% Initialize   $\overline{\mathbf{R}}\Big(\emptyset,\emptyset,\mathrm{Atk_{col}}(\mathcal{J})\Big) = \widetilde{\mathbf{R}}$;

\While{$cnt\leq t$}{
Initialize $\mathcal{P} = \emptyset$, $\mathcal{H} = \emptyset$;

Update the empirical joint distributions set $\widetilde{\mathcal{J}}$ using $\widetilde{\mathbf{R}}$;  %$\overline{\mathbf{R}}\Big(\emptyset,\emptyset,\mathrm{Atk_{col}}(\mathcal{J})\Big)$;

      \ForAll{\texttt{$p,q\in\mathcal{F}, p\neq q$}}{
      \ForAll{\texttt{$a\in[0,k_p-1], b\in[0,k_q-1]$}}{\If{$\big|J_{p,q}(a,b)-\widetilde{J_{p,q}}(a,b)\big| \geq \tau_{\mathrm{col}}^{\mathrm{Atk}}$}{
   $\mathcal{I} = \text{row\ index\ query}\big(\widetilde{\mathbf{R}}.p == a\ \text{and}\  \widetilde{\mathbf{R}}.q == b\big)$;  \\
   \ForAll{row index $i\in\mathcal{I}$}{
   
   \If{$\{i,p\}\notin\mathcal{P}$}{$\mathcal{P}=\mathcal{P}\cup \{i,p\}$;}
   
   
    \If{$\{i,q\}\notin\mathcal{P}$}{$\mathcal{P}=\mathcal{P}\cup \{i,q\}$;}
    
    % \CommentSty{//record new suspicious positions.}
    

   
   
   
   }
   }}
      
       }
       
   
\ForAll{ row index and attribute tuple  $\{i,p\}\in\mathcal{P}$}{


Collect all attributes   paired with row index $i$ into set $\mathcal{A}_i$

  
$\mathcal{H} = \mathcal{H} \cup \{i,\rm{mode}(\mathcal{A}_i)\}$;\CommentSty{//the most frequent attribute associate with row index $i$ is recorded in  $\mathcal{H}$.}\\}
     
     \ForAll{highly suspicious row index and attribute tuple $\{i,p\}\in\mathcal{H}$}   {\If{$\{i,p\}\notin\mathcal{Z}$}{Change the LSB of $\widetilde{\mathbf{R}}.(i,p)$;
     
     $\mathcal{Z} = \mathcal{Z}\cup \{i,p\}$;
     
    %  \CommentSty{//Append in $\mathcal{Z}$ to avoid repeated flipping in the following rounds.}\\
     
     
     }}
       
       $cnt = cnt+1;$
       
      % $\widetilde{\mathbf{R}}_{cnt}  = \widetilde{\mathbf{R}}_{cnt-1}$;
       
     }

     Return $\overline{\mathbf{R}}\Big(\emptyset,\emptyset,\mathrm{Atk_{col}}(\mathcal{J})\Big) = \widetilde{\mathbf{R}}$;
     
     
    %  Return $\overline{\mathbf{R}}\Big(\emptyset,\emptyset,\mathrm{Atk_{col}}(\mathcal{J})\Big)$.
     
     
		\caption{$\mathrm{Atk_{col}}(\mathcal{J})$: Column-wise Correlation     Attack}
	
\label{Algo:col-wise-attack}
\end{algorithm}
%, we summarize the steps to launch a  correlation-based   attack using prior knowledge on the  column-wise correlations obtain  from a publicly available database $\mathbf{R}_\kappa$.

{\color{black}
Next, we  show that a malicious SP can   increase its inference power (confidence) about whether  a particular entry in the database is fingerprinted or not by launching $\mathrm{Atk_{col}}(\mathcal{J})$. In Section \ref{sec:eva}, we   experimentally validate this finding using a real-world   database.  
Under  $\mathrm{Atk_{rnd}}$, we denote the malicious SP's confidence that an entry, whose attribute $p$ takes value $a$ in the original database ($\mathbf{R}$), is changed due to the fingerprinting as $\mathrm{Conf_{Atk_{rnd}}}(\frac{1}{\gamma};p,a)$.  
Likewise, under  $\mathrm{Atk_{col}}(\mathcal{J})$, we represent such confidence as $\mathrm{Conf_{Atk_{col}(\mathcal{J})}}(\frac{1}{\gamma};p,a)$. Here, $\gamma\in(0,1)$ is the fingerprinting ratio and we use $\frac{1}{\gamma}$ as the decision parameter to investigate the asymptotic behavior of  the malicious SP's confidence gain, which is defined  as the ratio  $G_{\mathrm{col}}(\frac{1}{\gamma};p,a) = {\mathrm{Conf_{Atk_{col}(\mathcal{J})}}(\frac{1}{\gamma};p,a)}\Big/{\mathrm{Conf_{Atk_{rnd}}}(\frac{1}{\gamma};p,a)}$. Thus, we have the following proposition. % (the proof sketch is shown in Appendix \ref{sec:supp_algos_col-wise-attack}).

\begin{prop}\label{prop:atk_col}
By launching $\mathrm{Conf_{Atk_{col}(\mathcal{J})}}$, the malicious SP's   confidence gain
% ($G_{\mathrm{col}}^*(p,a)$) 
about  an entry, whose attribute $p$ takes value $a$ in $\mathbf{R}$, is fingerprinted can be shown in an  asymptotic manner as
% \resizebox{1\hsize}{!}{$G_{\mathrm{col}}(\frac{1}{\gamma};p,a) = \frac{1-
%     \prod_{q\in\mathcal{T},q\neq p}\prod_{b\in[0,k_q-1]} \Pr\Big(\big|J_{p,q}(a,b)-\widetilde{J_{p,q}}(a,b)\big| < \tau_{\mathrm{col}}^{\mathrm{Atk}}\Big)}{\frac{\gamma}{|\mathcal{T}|}{freq}_{a}^p}$}\\$
%     = \Theta\vast(\Bigg({1-\prod_{q\in\mathcal{T},q\neq p}\Big(\frac{\tau_{\mathrm{col}}^{\mathrm{Atk}}}{\frac{\gamma}{|\mathcal{T}|}{2freq}_{a}^p}\Big)^{k_q}}\Bigg)\Bigg/\Bigg({\frac{\gamma}{|\mathcal{T}|}{freq}_{a}^p}\Bigg)\vast)$,\\
% where $= \frac{\gamma}{|\mathcal{T}|}{freq}_{a}^p,  p\in\mathcal{T}$, 
\begin{equation*}
    G_{\mathrm{col}}(\frac{1}{\gamma};p,a) 
    = \Theta\left(\left({1-\prod_{q\in\mathcal{T},q\neq p}\left(\frac{\tau_{\mathrm{col}}^{\mathrm{Atk}}}{\frac{\gamma}{|\mathcal{T}|}{2freq}_{a}^p}\right)^{k_q}}\right)\Bigg/\left({\frac{\gamma}{|\mathcal{T}|}{freq}_{a}^p}\right)\right),
\end{equation*}
where ${freq}_{a}^p$ is the frequency of records with attribute $p$ taking value $a$ in $\mathbf{R}$,   $k_q$ is the number of different values for attribute $q$, and $\Theta(\cdot)$ is the Big-Theta notation. 
\end{prop}
\begin{proof}[Proof Sketch] 
% Due to space limit, we only provide the proof sketch here. 
For the vanilla fingerprinting scheme, we have $\mathrm{Conf_{Atk_{rnd}}}(p,a)=\frac{\gamma}{|\mathcal{T}|}{freq}_{a}^p$. When launching the $\mathrm{Atk_{col}}(\mathcal{J})$, the malicious SP will add the corresponding suspicious row index and attribute tuple in $\mathcal{P}$ if $\big|J_{p,q}(a,b)-\widetilde{J_{p,q}}(a,b)\big| \geq \tau_{\mathrm{col}}^{\mathrm{Atk}}$. Thus, we have   $    \mathrm{Conf_{Atk_{col}(\mathcal{J})}}(p,a) = 1-
    \prod_{q\in\mathcal{T},q\neq p}\prod_{b\in[0,k_q-1]} \Pr\Big(\big|J_{p,q}(a,b)-\widetilde{J_{p,q}}(a,b)\big| < \tau_{\mathrm{col}}^{\mathrm{Atk}}\Big)$. Since the inserted fingerprint will cause  $J_{p,q}(a,b)-\widetilde{J_{p,q}}(a,b)$ vary in the range of $\Big[-\frac{\gamma}{|\mathcal{T}|}2freq_{a,b}^{p,q},\frac{\gamma}{|\mathcal{T}|}2 freq_{a,b}^{p,q}\Big]$, where $freq_{a,b}^{p,q}$ is the frequency of entries whose attributes $p$ and $q$ take values $a$ and $b$ in $\mathbf{R}$. 
    % we consider (assume?)
    Then, $|J_{p,q}(a,b)-\widetilde{J_{p,q}}(a,b)|$ can be shown as  a random variable attributed to an uniform distribution in the support of $\Big[0,\frac{\gamma}{|\mathcal{T}|}2 freq_{a,b}^{p,q}\Big]$, which leads to  $\mathrm{Conf_{Atk_{col}(\mathcal{J})}}(p,a) = 1- \prod_{q\in\mathcal{T},q\neq p}\prod_{b\in[0,k_q-1]} {\tau_{\mathrm{col}}^{\mathrm{Atk}}}\Big/\Big({\frac{\gamma}{|\mathcal{T}|}{2freq}_{a}^p} \Big)$. By applying   arithmetic-geometric mean inequality along with the fact   $\sum_{b\in[0,k_q-1]}freq_{a,b}^{p,q}  = freq_{a}^{p}, \forall q\neq p$, we can complete the proof.
% Since we known that $\sum_{b\in[0,k_q-1]}freq_{a,b}^{p,q}  = freq_{a}^{p}, \forall q\neq p$. By applying the arithmetic-geometric mean inequality, we have $1/\Big(\prod_{b\in[0,k_q-1]} {\frac{\gamma}{|\mathcal{T}|}{2freq}_{a,b}^{p,q}}\Big) \geq 1/(\frac{\gamma 2freq_a^p}{|\mathcal{T}|k_q})^{k_q}$, and hence, $\mathrm{Conf_{Atk_{col}(\mathcal{J})}}(p,a) \leq  1 - \prod_{q\in\mathcal{T},q\neq p}(\frac{\tau_{\mathrm{col}}^{\mathrm{Atk}}|\mathcal{T}|k_q}{\gamma 2freq_p^a})^{k_p}$, which concludes the proof.
% \begin{equation*}
% \begin{aligned}
%     &\mathrm{Conf_{Atk_{col}(\mathcal{J})}}(p,a) \\
%     =& 1-
%     \prod_{q\in\mathcal{T},q\neq p}\prod_{b\in[0,k_q-1]} \Pr\Big(\big|J_{p,q}(a,b)-\widetilde{J_{p,q}}(a,b)\big| < \tau_{\mathrm{col}}^{\mathrm{Atk}}\Big)
%     \end{aligned}
% \end{equation*}
\end{proof}
\begin{remark}
We aim at presenting a generic confidence gain achieved from $\mathrm{Atk_{col}}(\mathcal{J})$, thus we consider the potential fingerprinted entries in the suspicious set $\mathcal{P}$ instead of the highly suspicious set $\mathcal{H}$. In practice, the generation process of  $\mathcal{H}$ from $\mathcal{P}$ heavily depends on the data distribution in the considered databases. %In Section \ref{sec:theory_validate}, we will further interpret $G_{\mathrm{col}}(\frac{1}{\gamma};p,a)$ by plotting its analytical values under varying $\gamma$ and compare them with the empirical values.  
% impossible to use approximated mathematical models to accurately capture
\end{remark}

}













\subsection{Row-wise Correlation Attack}
\label{sec:row-wise-atack}

% \ea{We need the written description of the algorithm as well}

Since the malicious SP has access to both individuals' memberships to   communities and row-wise correlations, i.e.,  $\mathcal{S}$, 
% \hl{EA: this has a different representation in the table}, 
after receiving the fingerprinted database, it can compute a new set of statistical relationships 
% \hl{EA: we try to describe this as row-wise correlation attack but instead of correlations, we use similarities. To be consistent, I think we should use correlations everywhere (also in the notation table)} 
among pairs of individuals in each of the communities using $\widetilde{\mathbf{R}}$, %\footnote{We assume that the added fingerprint does not change individuals' memberships.} 
i.e.,  $\widetilde{\mathcal{S}} =  \{\widetilde{s_{ij}}^{\mathrm{comm}_c}|i,j\in\mathrm{comm}_c, i\neq j, c\in[1,C]\}$, where $\widetilde{s_{ij}}^{\mathrm{comm}_c} = e^{-\mathrm{dist}(\widetilde{\boldsymbol{r}_i},\widetilde{\boldsymbol{r}_j})}$ is the statistical relationship between the $i$th and $j$th data records (i.e., $\widetilde{\boldsymbol{r}_i}$ and $\widetilde{\boldsymbol{r}_j}$) in $\widetilde{\mathbf{R}}$. 
% \hl{EA: if you add an index to r (as I noted before), you can represent these as $\boldsymbol{r}_i$ and $\boldsymbol{r}_j$} in community $\mathrm{comm}_c$ after fingerprinting.
%Then, the malicious SP conducts row-wise correlation-based attack by flipping the LSB of all attributes of data records $i$ and $j$ if 
Then, to conduct $\mathrm{Atk_{row}}(\mathcal{S})$, the malicious SP flips the LSBs of all attributes of a   data record $\boldsymbol{r}_i$, 
%\hl{EA: use $\boldsymbol{r}_i$, also for the rest of the discussion as well}, 
if the cumulative absolute difference of its  statistical relationships with respect to other records in the same community exceeds a predetermined threshold $\tau_{\mathrm{row}}^{\mathrm{Atk}}$ after fingerprinting, i.e., $\sum_{j\neq i}^{n_c} \   \big|s_{ij}^{\mathrm{comm}_c}-\widetilde{s_{ij}}^{\mathrm{comm}_c}\big| \geq \tau_{\mathrm{row}}^{\mathrm{Atk}}, i,j\in\mathrm{comm}_c$.   {\color{black} The rationale behind this is because the row-wise statistical information $\mathcal{S}$ is calculated using  the entire data records, instead of individual entries between the rows. Although, this represents the strongest row-wise attack as it changes all the entries of a given data record, in practice, $\mathrm{Atk_{row}(\mathcal{S})}$ changes only a limited number of data records, as will be shown in Section \ref{sec: int_attack_census}.} We summarize the steps to launch $\mathrm{Atk_{row}}(\mathcal{S})$ on $\widetilde{\mathbf{R}}$ in Algorithm \ref{algo:row-wise-attack}. % in Appendix~\ref{sec:supp_algos_row-wise-attack}.

\begin{algorithm}
\small
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Fingerprinted database, $\widetilde{\mathbf{R}}$, malicious SP's prior knowledge on the row-wise correlations  $\mathcal{S}$ and individuals' affiliation to the $C$ communities.}
\Output{$\overline{\mathbf{R}}\Big(\emptyset,\mathrm{Atk_{row}}(\mathcal{S}),\emptyset,\Big)$.}

% Initialize $\overline{\mathbf{R}}\Big(\emptyset,\mathrm{Atk_{row}}(\mathcal{S}),\emptyset,\Big) = \widetilde{\mathbf{R}}$;

Obtain  the new set of  pairwise statistical relationships among individuals in each community   from  $\widetilde{\mathbf{R}}$, i.e., $\widetilde{\mathcal{S}}$;

\ForAll{$\mathrm{comm}_c, c\in[1,C]$}{\ForAll{individual $i\in \mathrm{comm}_c$}{\If{$\sum_{j\neq i}^{n_c} \   \big|s_{ij}^{\mathrm{comm}_c}-\widetilde{s_{ij}}^{\mathrm{comm}_c}\big| \geq \tau_{\mathrm{row}}^{\mathrm{Atk}}$}{Flip the LSBs of all attributes of $\boldsymbol{r}_i$ in $\widetilde{\mathbf{R}}$;}

}}


 
 Return $\overline{\mathbf{R}}\Big(\emptyset,\mathrm{Atk_{row}}(\mathcal{S}),\emptyset,\Big) = \widetilde{\mathbf{R}}$.

		\caption{$\mathrm{Atk_{row}}(\mathcal{S})$: Row-wise correlation  attack}
\label{algo:row-wise-attack}
\end{algorithm}




% We also analyze the impact of $\mathrm{Atk_{row}}(\mathcal{S})$. 

% $\mathrm{Atk_{row}}(\mathcal{S})$ changes all entries of identified data records, thus,  
We analyze the impact of $\mathrm{Atk_{row}}(\mathcal{S})$ by denoting the malicious SP's confidence that an entry ($\boldsymbol{r}_i$) is fingerprinted as $\mathrm{Conf}_{\mathrm{Atk_{rnd}}}(\frac{1}{\gamma};\boldsymbol{r}_i)$ and $\mathrm{Conf}_{\mathrm{Atk_{row}}(\mathcal{S})}(\frac{1}{\gamma};\boldsymbol{r}_i)$, under $\mathrm{Atk_{rnd}}$ and $\mathrm{Atk_{row}}(\mathcal{S})$, respectively. Then, 
% similarly, we let such confidence after launching $\mathrm{Atk_{row}}(\mathcal{S})$ be $\mathrm{Conf}_{\mathrm{Atk_{row}}(\mathcal{S})}(\frac{1}{\gamma};\boldsymbol{r}_i)$, and define 
the confidence  gain of the malicious SP is  $G_{\mathrm{row}}(\frac{1}{\gamma};\boldsymbol{r}_i) = \frac{\mathrm{Conf}_{\mathrm{Atk_{row}}(\mathcal{S})}(\frac{1}{\gamma};\boldsymbol{r}_i)}{\mathrm{Conf}_{\mathrm{Atk_{rnd}}}(\frac{1}{\gamma};\boldsymbol{r}_i)}$, which is calculated in the following proposition.



\begin{prop}\label{prop:atk-row}
By launching $\mathrm{Conf_{Atk_{row}(\mathcal{S})}}$, the malicious SP's maximum confidence gain  about  an entry   in $\mathbf{R}$ is fingerprinted can be shown asymptotically as  
\begin{equation*}
    G_{\mathrm{row}}(\frac{1}{\gamma};\boldsymbol{r}_i)  = \Theta\vast( \Bigg(1-\sum_{j=0}^{\floor*{\tau_{\mathrm{row}}^{\mathrm{Atk}}}}{n_c-1 \choose j}(2\gamma-\gamma^2)^j(1-\gamma)^{2(n_c-1-j)}\Bigg)  \Big/ \gamma \vast).
\end{equation*}
\end{prop}
\begin{proof}[Proof Sketch]
Clearly, $\mathrm{Conf}_{\mathrm{Atk_{rnd}}}(\boldsymbol{r}_i) = \gamma$. 
According to Algorithm \ref{algo:row-wise-attack},  $\mathrm{Conf}_{\mathrm{Atk_{row}}(\mathcal{S})}(\frac{1}{\gamma};\boldsymbol{r}_i) = \Pr(\sum_{j\neq i}^{n_c} \   \big|e^{-\mathrm{dist}(\boldsymbol{r}_i,\boldsymbol{r}_j)}-e^{-\mathrm{dist}(\widetilde{\boldsymbol{r}_i},\widetilde{\boldsymbol{r}_j})}\big| \geq \tau_{\mathrm{row}}^{\mathrm{Atk}})\stackrel{*}\approx \Pr(\sum_{j\neq i}^{n_c} \   \big|\mathrm{dist}(\boldsymbol{r}_i,\boldsymbol{r}_j)-\mathrm{dist}(\widetilde{\boldsymbol{r}_i},\widetilde{\boldsymbol{r}_j})\big| \geq \tau_{\mathrm{row}}^{\mathrm{Atk}})$, where $*$ is due to the Taylor approximation and the assumption that the distance between individuals in the same community is   small. Then,  $|\mathrm{dist}(\boldsymbol{r}_i,\boldsymbol{r}_j)-\mathrm{dist}(\widetilde{\boldsymbol{r}_i},\widetilde{\boldsymbol{r}_j})\big|$ can be shown as a Bernoulli  random variable, which is $0$ with probability $(1-\gamma)^2$, and is nonzero with probability $2\gamma-\gamma^2$. Since the summation of Bernoulli random variable is attributed to binomial distribution, we can finish the proof.
\end{proof}
\begin{remark}
In the above analysis, we   ignored the scenario where $|\mathrm{dist}(\boldsymbol{r}_i,\boldsymbol{r}_j)-\mathrm{dist}(\widetilde{\boldsymbol{r}_i},\widetilde{\boldsymbol{r}_j})\big|$ is $2$ with probability $\gamma^2$ to avoid extra heavy notations. In the experiments, we set $\gamma=1/35$, thus, $\gamma^2$ is negligible. %In Section \ref{sec:theory_validate}, we have shown that the analytical values of $    G_{\mathrm{row}}(\frac{1}{\gamma};\boldsymbol{r}_i) $ are close to the empirical values.
\end{remark}


% \subsection{A Toy Example?}

%\ea{Is this going to be dataset dependent? lets discuss about this}


% \hl{EA: you have a discussion (in the evaluation) about how these 2 attacks can be combined by the attacker. Can you move it to here and maybe extend it if needed?}

% \hlgreen{TJ: then, do we also mention the dataset for this result here? or refer to it in later sections?} \hl{EA: no, I think you should make that discussion independent of the dataset}



\subsection{Integrated Correlation Attack}
\label{sec:effect_corr_attack}

In practice, the malicious SP will apply $\mathrm{Atk_{row}}(\mathcal{S})$ followed by $\mathrm{Atk_{col}}(\mathcal{J})$ if it launches the integrated correlation attack. {\color{black}This is because  (i) $\mathrm{Atk_{row}}(\mathcal{S})$ is computationally light and  modifies significantly  less entries in $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$ compared to $\mathrm{Atk_{col}}(\mathcal{J})$ (as we will show in Section~\ref{sec: int_attack_census}). (ii) If $\mathrm{Atk_{col}}(\mathcal{J})$ is applied first, it will change   the row-wise correlations ($\mathrm{P_{row}}$)  significantly, yet, if $\mathrm{Atk_{row}}(\mathcal{S})$ is applied first, it only has a small impact on the column-wise correlations $\mathrm{P_{col}}$ (as we will also show in Section~\ref{sec: int_attack_census}).}  Algorithm \ref{algo:int-attack}    summarizes the major steps of this integrated attack. Note that, in practice,  there is no  minimum distribution difference requirement  to perform the proposed attacks, because a malicious SP can always reduce the value of  $\tau_{\mathrm{col}}^{\mathrm{Atk}}$ and $\tau_{\mathrm{row}}^{\mathrm{Atk}}$ to obtain more potentially fingerprinted entries.

\begin{algorithm}
\small
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Fingerprinted database, $\widetilde{\mathbf{R}}$, malicious SP's prior knowledge on the row-wise correlations  $\mathcal{S}$, individuals' affiliation to the $C$ communities, and column-wise correlations  $\mathcal{J}$.}
\Output{$\overline{\mathbf{R}}\Big(\emptyset,\mathrm{Atk_{row}}(\mathcal{S}),\mathrm{Atk_{col}}(\mathcal{J})\Big)$.}

% Initialize $\overline{\mathbf{R}}\Big(\emptyset,\mathrm{Atk_{row}}(\mathcal{S}),\mathrm{Atk_{col}}(\mathcal{J})\Big) = \widetilde{\mathbf{R}}$;

Launch row-wise correlation attack   $\mathrm{Atk_{row}}(\mathcal{S})$ on $\widetilde{\mathbf{R}}$ using Algorithm \ref{algo:row-wise-attack}, and obtain $\overline{\mathbf{R}}\Big(\emptyset,\mathrm{Atk_{row}}(\mathcal{S}),\emptyset\Big)$;

Launch  column-wise correlation attack  $\mathrm{Atk_{col}}(\mathcal{J})$ on $\overline{\mathbf{R}}\Big(\emptyset,\mathrm{Atk_{row}}(\mathcal{S}),\emptyset\Big)$ using Algorithm \ref{Algo:col-wise-attack}, obtain and return   $\overline{\mathbf{R}}\Big(\emptyset,\mathrm{Atk_{row}}(\mathcal{S}),\mathrm{Atk_{col}}(\mathcal{J})\Big)$.

\caption{Integrated correlation attack}
\label{algo:int-attack}
\end{algorithm}



% Thus, in practice, the malicious SP will apply $\mathrm{Atk_{row}}(\mathcal{S})$ followed by $\mathrm{Atk_{col}}(\mathcal{J})$ if it launches the integrated correlation attack. In Algorithm \ref{algo:int-attack} we summarize the major steps of this integrated attack. 






% \hl{EA: lets just call them "correlation attacks" not "correlation-based attacks}



By taking advantage of the correlation models, the identified attacks (in Sections \ref{sec:col-wise-attack} and \ref{sec:row-wise-atack}) are   more powerful than the traditional random bit flipping attack  (in Section \ref{sec:threat_models}). As we will show in Section~\ref{sec: int_attack_census}, to effectively distort the added fingerprint and cause Alice to accuse innocent SPs with high probability, a malicious SP only needs to change a small fraction of entries in the fingerprinted database if it conducts the correlation attacks  on $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$. 
In contrast, to achieve a similar attack performance, the random bit flipping attack   needs to change  more than $80\%$ of the entries in $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$, which results in a significant loss in     database utility. Thus, the   correlation attacks not only distort the inserted fingerprint but they also maintain a high utility for the pirated database.  
%Thus, we will also validate that by changing less entries, the attacked fingerprinted database (i.e., $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\mathrm{Atk_{row}}(\mathcal{S}),\mathrm{Atk_{col}}(\mathcal{J})\Big)$, $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\mathrm{Atk_{row}}(\mathcal{S})\Big)$, or $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\mathrm{Atk_{col}}(\mathcal{J})\Big)$) can achieve higher utility in terms of several different utility metrics, 
%such as accuracy and    column- and row-wise correlation preservation. 

Due to the identified vulnerability of existing fingerprinting schemes for relations against correlation attacks, it is critical to develop defense mechanisms that can mitigate these attacks. In the next section, we discuss how to develop robust fingerprinting techniques against both column- and row-wise correlation attacks. 


\section{Robust Fingerprinting Against Identified Correlation Attacks}
\label{sec:robust_fp}


Now, we propose robust fingerprinting schemes against the identified correlation attacks that can serve as post-processing steps for any off-the-shelf (vanilla) fingerprinting schemes.  
% \hl{EA: for J and S, I think we should use the input arguments (as in the notations table). It is important from which dataset they are computed.}
To provide robustness against column- and row-wise correlation attack, i.e.,  $\mathrm{Atk_{col}(\mathcal{J})}$ and   $\mathrm{Atk_{row}(\mathcal{S})}$, the database owner (Alice) utilizes her prior knowledge $\mathcal{J}'$ and $\mathcal{S}'$ as the reference column-wise joint distributions and statistical relationships, respectively. We will show that to implement the proposed mitigation techniques, Alice needs to change only a few entries (e.g., less than $3\%$) in $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$, 
% \hl{EA: notation not consistent with the table, lets keep the input arguments fixed}, 
such that the post-processed fingerprinted database has    column-wise correlation    close to $\mathcal{J}'$ and row-wise correlation     far from  $\mathcal{S}'$.
% In practice,  $\mathcal{J}'$ and $\mathcal{S}'$ may be different from $\mathcal{J}$ and $\mathcal{S}$, which are used by   the malicious SP  to launch correlation attacks. For example, $\mathcal{J}'$ and $\mathcal{S}'$ can be directly calculated from the original database $\mathbf{R}$ \hl{EA: we said J and S are calculated directly from the dataset before, right? If so, this is confusing}, which is only available to the database owner, or they can be obtained by the database owner from a  resource that is different with the malicious SP. We refer to this as prior knowledge asymmetry between database owner and malicious SP, and we will empirically evaluate its impact on attacks and defenses in fingerprinted databases in Section \ref{.}

%\hl{EA: you can add something like "to the advantage of the malicious SP, we assume the malicious SP always has more accurate or at least equally accurate knowledge about column-wise joint distributions and row-wise statistical relationships}


\subsection{Robust Fingerprinting Against Column-wise Correlation Attack}
\label{sec:col_defense}

% \hl{EA: as mentioned before, I think when you dont write the input arguments for J, J', etc, it becomes confusing. Based on the notation table both J and J' can be denoted in the same way with different datasets as the input arguments; for J, input argument can be R, for J', input argument can be a noisy version of R.}

\subsubsection{Mitigation via mass transportation} 
To make a vanilla fingerprinting scheme robust against column-wise correlation attack, the main goal of the proposed technique   $\mathrm{Dfs_{col}}(\mathcal{J}')$ is to transform  $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$ to have column-wise joint distributions close to  the reference joint distributions in $\mathcal{J}'$. We develop  $\mathrm{Dfs_{col}}(\mathcal{J}')$ using ``optimal transportation''~\cite{courty2016optimal}, which moves the probability  mass of the marginal distribution of each attribute in $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$ to resemble the distribution obtained from the marginalization of each reference joint distribution in $\mathcal{J}'$. Then, the optimal transportation plan is used to change the entries in each attribute of  $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$ to obtain $\widetilde{\mathbf{R}}\big(\mathrm{FP},\emptyset,\mathrm{Dfs_{col}}(\mathcal{J}')\big)$. 
% By making the marginal distribution of each attribute close to that obtained from   marginalizing  the reference joint distribution in $\mathcal{J}'$,
While doing this, the new empirical joint distributions calculated from     $\widetilde{\mathbf{R}}\big(\mathrm{FP},\emptyset,\mathrm{Dfs_{col}}(\mathcal{J}')\big)$ also become close to the ones in  $\mathcal{J}'$. %\footnote{\hlgreen{TJ:may delete this footnote...} Note that even if the marginal distributions on attribute $p$ and $q$ obtained from $\widetilde{\mathbf{R}}(\mathrm{FP},\mathrm{Dfs_{col}}(\mathcal{J}'))$ are identical with the marginal distributions obtained from marginalization of $J_{p,q}$ in $\mathcal{J}$, the empirical joint distribution obtained from $\widetilde{\mathbf{R}}(\mathrm{FP},\mathrm{Dfs_{col}}(\mathcal{J}'))$ may still be different from $J_{p,q}$, because the joint distribution with specific marginal distributions are not unique. Even then, the developed $\mathrm{Dfs_{col}(\mathcal{J})'}$ is robust against $\mathrm{Atk_{col}(\mathcal{J})}$, as will be shown in  Section \ref{}. We will elaborate why we do not directly move the mass of joint distributions to make them identical to those in $\mathcal{J}'$ and discuss the advantage of our design in  Section \ref{sec:adv_col_dfs}.}  
% {\color{black}Even if $\mathcal{J}'$ is different from $\mathcal{J}$, which is utilized by the malicious SP, we show (in Section~\ref{sec:eva}) that $\mathrm{Dfs_{col}}(\mathcal{J}')$ can still mitigate $\mathrm{Atk_{col}}(\mathcal{J})$. Thus, the malicious SP can still be accused with high probability (i.e., either uniquely accusable or with a high accusable ranking $r$) if it leaks a copy of   $\widetilde{\mathbf{R}}\big(\mathrm{FP},\emptyset,\mathrm{Dfs_{col}}(\mathcal{J}')\big)$.}


% If $\mathcal{J}'$ is the same or close to $\mathcal{J}$, which is utilized by the malicious SP, then the malicious SP will not be able to identify enough suspicious fingerprinted entries when launching $\mathrm{Atk_{col}}(\mathcal{J})$. As a result, the malicious SP will be accused if it leaks a copy of   $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\emptyset,\mathrm{Dfs_{col}}(\mathcal{J}')\Big)$. %We will experimentally corroborate this in Section \ref{}.


In particular, for a specific attribute (column) $p$, we denote its marginal distribution obtained from the (vanilla) fingerprinted database as $\Pr(C_{\widetilde{p}})$, and that obtained from the  marginalization of a reference $J'_{p,q}$ distribution in $\mathcal{J}'$ as $\Pr(C_{p'}) = J'_{p,q}\mathbf{1}^T$ ($q$ can be any attribute that is different from $p$, because the marginalization with respect to $p$ using different $J'_{p,q}$ will lead to the identical marginal distribution of $p$).
% \hl{EA: we can probably obtain many different marginal distribution for p using marginalization of different joint distributions. Which one do we end up using?}. 
To move the mass of $\Pr(C_{\widetilde{p}})$ to resemble $\Pr(C_{p'})$, we need to find another joint distribution (i.e., the mass transportation plan)  $G_{\widetilde{p},p'}\in\R^{k_p\times k_p}$ ($k_p$ is the number of possible values that attribute $p$ can take), whose marginal distributions are identical to $\Pr(C_{\widetilde{p}})$ and $\Pr(C_{p'})$. 
% \hl{EA: the way we use a and b below is not very clear to me}
Let $a$ and $b$ be two distinct values that attribute $p$ can take ($a,b\in[0,k_p-1]$). Then,  $G_{\widetilde{p},p'}(a,b)$ indicates that the database owner should change $G_{\widetilde{p},p'}(a,b)$ percentage of entries in $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$ whose attribute $p$ takes value $a$ (i.e., $p=a$) to value $b$ (i.e., change them to make $p=b$), so as to  make $\Pr(C_{\widetilde{p}})$ close to $\Pr(C_{p'})$. In practice, such a transportation plan can be obtained by solving a regularized optimal transportation problem, i.e., the entropy regularized Sinkhorn distance minimization  \cite{cuturi2013sinkhorn} as follows:  
% \begin{equation}
% \label{ot_defense}
% \begin{aligned}
% &d\Big(\Pr(C_{\widetilde{p}}),\Pr(C_{p'}),\lambda_p\Big) \\
% =& \min_{G_{\widetilde{p},p'}\in\mathcal{G}\big(\Pr(C_{\widetilde{p}}),\Pr(C_{p'})\big)}<G_{\widetilde{p},p'},\Theta_{\widetilde{p},p'}>_F-\frac{H(G_{\widetilde{p},p'})}{\lambda_{p}},
% \end{aligned}
% \end{equation}
% \setlength{\abovedisplayskip}{3pt}
% \setlength{\belowdisplayskip}{3pt}
\begin{equation}
\label{ot_defense}
\begin{aligned}
&d\Big(\Pr(C_{\widetilde{p}}),\Pr(C_{p'}),\lambda_p\Big) \\
&= \min_{G_{\widetilde{p},p'}\in\mathcal{G}\big(\Pr(C_{\widetilde{p}}),\Pr(C_{p'})\big)}<G_{\widetilde{p},p'},\Theta_{\widetilde{p},p'}>_F-\frac{H(G_{\widetilde{p},p'})}{\lambda_{p}},
\end{aligned}
\end{equation}
where     $\mathcal{G}\big(\Pr(C_{\widetilde{p}}),\Pr(C_{p'})\big) = \big\{G\in\R^{k_p\times k_p}\big|G\mathbf{1} = \Pr(C_{\widetilde{p}}),G^T\mathbf{1}  = \Pr(C_{p'})\big\}$ is the set of all  joint probability distributions whose marginal distributions are the probability mass functions   of  $\Pr(C_{\widetilde{p}})$ and $\Pr(C_{p'})$. $<\cdot,\cdot>_F$ denotes the Frobenius inner product 
% (summation of     element-wise products) 
of two matrices with the same size. Also, $\Theta_{\widetilde{p},p'}$ is the transportation cost matrix and $\Theta_{\widetilde{p},p'}(a,b)>0$ represents the cost to move a unit percentage of mass from $\Pr(C_{\widetilde{p}} = a)$ to $\Pr(C_{\widetilde{p}} = b)$. Finally, $H(G_{\widetilde{p},p'}) = -<G_{\widetilde{p},p'},\log G_{\widetilde{p},p'}>_F$ calculates  the information entropy of $G_{\widetilde{p},p'}$ and $\lambda_p>0$ is a tuning parameter. In practice, (\ref{ot_defense}) can be solved by iteratively rescaling rows and columns of the initialized $G_{\widetilde{p},p'}$ to have desired marginal distributions.  The obtained $G_{\widetilde{p},p'}$ is more heterogeneous for larger values of $\lambda_p$. This suggests that the transportation plan 
tends to move the mass of 
$\Pr(C_{\widetilde{p}} = a)$ to the adjacent instances, i.e, $b=a-1$ or $b=a+1$. In contrast, the obtained $G_{\widetilde{p},p'}$ is more homogeneous for smaller values of $\lambda_p$, which suggests that the transportation plan tends to move the mass of 
$\Pr(C_{\widetilde{p}} = a)$ to all other instances.  {\color{black}A  homogeneous plan makes   $\Pr(C_{\widetilde{p}})$ much closer to $\Pr(C_{p'})$ after the mass transportation, but it causes more data entries to be changed, and results in a higher decrease in the database utility. On the other hand, a heterogeneous plan changes less data entries by tolerating a larger difference between  $\Pr(C_{\widetilde{p}})$ and $\Pr(C_{p'})$ after the mass transportation. In the evaluation (in Section~\ref{sec:eva}), we will try different values of  $\lambda_p$ to strike a balance between the mitigation performance and data utility.} 


% In Appendix~\ref{sec:toy_example}, we show a toy example to illustrate $\mathrm{Dfs_{col}}(\mathcal{J}')$ via mass transportation of $\Pr(C_{\widetilde{p}})$ to resemble $\Pr(C_{p'})$.
 



\subsubsection{A toy example on mass transportation}
\label{sec:toy_example}
To illustrate $\mathrm{Dfs_{col}}(\mathcal{J}')$ via mass transportation of $\Pr(C_{\widetilde{p}})$ to resemble $\Pr(C_{p'})$, we use a pair of discrete probability distributions shown in Figure \ref{fig:OT_toy_example}(a) as an example, and demonstrate the transportation plans obtained by solving (\ref{ot_defense}) when $\lambda_p=500$ and $\lambda_p=50$ in Figures \ref{fig:OT_toy_example}(b) and (c), respectively.
% \hl{EA: if the table is only related to the toy example, can you make the table a part of the figure and show them together? (I mean embed the table in the figure and just call it a single figure)} 
In Figure \ref{fig:OT_toy_example}(b), we have a heterogeneous  $G_{\widetilde{p},p'}$, which often  moves the mass to adjacent instances, e.g., the mass of $\Pr(C_{\widetilde{p}}=0)$ is divided into 3 parts and a larger portion of mass is moved to $\Pr(C_{\widetilde{p}}=1)$.    $G_{\widetilde{p},p'}(0,1) = 0.157$,  thus $0.157$ mass  of $\Pr(C_{\widetilde{p}}=0)$ is moved to $\Pr(C_{\widetilde{p}}=1)$.  In Figure~\ref{fig:OT_toy_example}(c), we obtain a homogeneous $G_{\widetilde{p},p'}$, which distributes the mass to many other instances. For example, the mass of $\Pr(C_{\widetilde{p}}=0)$ is divided into 5 parts and 4 of them are  moved to $\Pr(C_{\widetilde{p}}=1)$, $\Pr(C_{\widetilde{p}}=2)$, $\Pr(C_{\widetilde{p}}=3)$, and $\Pr(C_{\widetilde{p}}=5)$. 


\begin{figure}[htb]
  \begin{center}
     \includegraphics[width= 0.7\columnwidth]{figures/OT_example.jpg}
      \end{center}
  \caption{\label{fig:OT_toy_example} Visualization of mass transportation plans obtained by solving (\ref{ot_defense}) using different $\lambda_p$ values to move   mass of $\Pr(C_{\widetilde{p}})$ to resemble $\Pr(C_{p'})$. (a) example discrete probability distributions. (b) if $\lambda_p=500$, we achieve a heterogeneous plan, which tolerates more   difference between  $\Pr(C_{\widetilde{p}})$ and $\Pr(C_{p'})$ after the mass transportation. 
  (c) if $\lambda_p=50$, we achieve a homogeneous plan. which makes    $\Pr(C_{\widetilde{p}})$ more closer to $\Pr(C_{p'})$ after the mass transportation.
}
\end{figure}





% \subsubsection{Utility preservation} \hl{TJ: I will revise the following two subsections} As discussed in Section \ref{sec:vanilla}, to preserve the utility  of the fingerprinted database, database owner (Alice) only changes the LSB of selected entries when applying the vanilla  fingerprinting scheme.
% % \hl{EA: is this true for the vanilla scheme or only for our proposed ad on?}. 
% % \hlgreen{TJ: when we implement vanilla, it will also just change the LSB of entries. We will show this can lead to high utility.} 
% Similarly, she also needs to consider this utility constraint when implementing $\mathrm{Dfs_{col}}(\mathcal{J}')$. To do this, given a transportation plan, Alice moves the mass of an instance only to the two instances that can be obtained by changing the LSB of that instance, e.g., moving the mass of  $\Pr(C_{\widetilde{p}}=1)$ to $\Pr(C_{\widetilde{p}}=0)$ and $\Pr(C_{\widetilde{p}}=2)$ if $p$ has more than 3 instances. 
% % \hl{EA: if you consider these as binary entries, how do you obtain a 2 by changing the LSB of a 0? you need to change the last 2 bits for that, right?}. 
% We refer to such a moves as ``LSB-approved transportation'' (i.e., green solid arrows in Figure~\ref{fig:OT_toy_example}), and all other moves are called ``LSB-denied  transportations'' (i.e., red dashed  arrows in Figure~\ref{fig:OT_toy_example}). Note that if an attribute only has 2 instances (i.e., binary entries such as sex), all moves will be LSB-approved transportation, but transportation  plan obtained with   higher $\lambda_p$ will change less entries in the database and preserve more utility. 




\subsubsection{Algorithm description} In the following, we formally describe the procedure of $\mathrm{Dfs_{col}}(\mathcal{J}')$. After Alice generates $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$ using the vanilla fingerprinting scheme, she   evaluates the new  joint distributions of all pairs of attributes, i.e., $\widetilde{J_{p,q}}, p,q\in\mathcal{F},p\neq q$, and compares them  with the reference joint distributions   $\mathcal{J}_{p,q}',  p,q\in\mathcal{F},p\neq q$.
% \hl{EA: same comment as before}. 
If the discrepancy between a particular pair of joint distributions exceeds a predetermined threshold, i.e., 
%  \hl{EA: dont use such terms for measurement, use concrete terms}  
 $||\widetilde{J_{p,q}}-J'_{p,q}||_F\geq \tau_{\mathrm{col}}^{\mathrm{Dfs}}$, Alice records both attributes $p$ and $q$ in a set $\mathcal{Q}$. 
%  \hl{EA: didnt we use I for this set for the attack? Maybe you can use a similar symbol again here}. \hlgreen{TJ: in attack, we use I to record the row indices}
For all the attributes in $\mathcal{Q}$, Alice obtains $\Pr(C_{\widetilde{p}})$ from $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset).p$ 
% \hl{EA: did you introduce $.p$ notation before?} 
and calculates $\Pr(C_{p'}) = J'_{p,q}\mathbf{1}^T$. Next, she gets the optimal transportation plan for attribute $p$  
by solving (\ref{ot_defense}). Then, she changes the instances  of $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset).p$ to other instances by following the 
transportation moves suggested by   $G_{\widetilde{p},p'}$, i.e., given $G_{\widetilde{p},p'}(a,b)$,  Alice randomly samples $G_{\widetilde{p},p'}(a,b)$ fraction of entries (excluding the fingerprinted entries) whose attribute $p$ takes value $a$ and changes them to $b$.   We summarize the procedure of $\mathrm{Dfs_{col}}(\mathcal{J}')$ in Algorithm \ref{algo:ot_defense}, where lines \ref{line:ot_start}-\ref{line:ot_end} solves (\ref{ot_defense}) to obtain the optimal mass transportation plan for attribute $p$, and lines \ref{line:move_start}-\ref{line:move_end} change the values of entries in $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset).p$ according to $G_{\widetilde{p},p'}$.

\begin{algorithm}[htb]
\small
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Vanilla fingerprinted database  $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$, locations  of entries changed by the vanilla fingerprinting  scheme, and Alice's prior knowledge on the   joint distributions of the pairwise attributes, i.e.,  $\mathcal{J}'$.}
\Output{$\widetilde{\mathbf{R}}\Big(\mathrm{FP},\emptyset,\mathrm{Dfs_{col}}(\mathcal{J}')\Big)$.}

Initialize $\mathcal{Q}=\emptyset$;

Obtain the empirical joint distributions set $\widetilde{\mathcal{J}}$ using $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$;

\ForAll{$p,q\in\mathcal{F},p\neq q$}{\If{$||J'_{p,q}-\widetilde{J}_{p,q}||_F>\tau_{\mathrm{col}}^{\mathrm{Dfs}}$}{$\mathcal{Q} = \mathcal{Q}\cup p \cup q$;}}

\ForAll{$p\in\mathcal{Q}$}{

Initialize the mass movement cost matrix $\Theta_{\widetilde{p},p'}$ and tuning parameter $\lambda_p$;\label{line:ot_start}

Obtain empirical marginal  distribution $\Pr(C_{\widetilde{p}})$ from $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset).p$;

       Initialize $G_{\widetilde{p},p'} = e^{-\lambda_{p}\Theta_{\widetilde{p},p'}}$; 
        
\While{not converge}{
Scale the rows of $G_{\widetilde{p},p'}$ to make  the rows sum to the marginal distribution $\Pr(C_{\widetilde{p}})$;

Scale the columns of $G_{\widetilde{p},p'}$ to make the columns sum to the marginal distribution $\Pr(C_{p'})$;
}\label{line:ot_end}
 
 \ForAll{$a\in[0,k_p-1]$\label{line:move_start}}{\ForAll{$b\in [0,k_p-1], b\neq a$}{Sample $G_{\widetilde{p},p'}(a,b)$ percentage of entries from $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset).p$ (excluding the vanilla  fingerprinted entries) whose attribute $p$ takes value $a$, and change their value to $b$;}
 
 
 }\label{line:move_end}
 
 
 }
 
 Return $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\emptyset,\mathrm{Dfs_{col}}(\mathcal{J}')\Big)$.

		\caption{$\mathrm{Dfs_{col}}(\mathcal{J}')$: defense against column-wise correlation   attack.}
\label{algo:ot_defense}
\end{algorithm}


% {\color{blue}In Section \ref{sec:col-wise-attack}, we have theoretically analyzed the attack-ability of $\mathrm{Atk_{col}}$ in terms of $G_{\mathrm{col}}(\frac{1}{\gamma};p,a)$, similarly technique can also be applied to analyze the defense-ability of $\mathrm{Dfs_{col}}$ by investigating the differences between the malicious SP's prior knowledge $\mathcal{J}$ and the optimal solution to (\ref{ot_defense}). We will explore this  in the future work.}
% In Appendix~\ref{sec:supp_design_detail_of_dfs_col}, we elaborate more on the design details of $\mathrm{Dfs_{col}}(\mathcal{J}')$ and explain why we do not  apply the optimal transportation technique to directly move the mass of the joint distributions obtained from $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$ to resemble the joint distributions in  $\mathcal{J}'$. 



% LSB-approved 
% % \hl{EA: do you mean LSB-based?}
% transportation moves in  $G_{\widetilde{p},p'}$ (which only change the LSB of entries). 
% % \hl{EA: if general (entire paper) you use a and b to give examples, but sometimes it is not clear where this a and b comes. We can discuss about this}
% We denote the set of instances that can be obtained by changing the LSB of a value $a$ as $\mathcal{LSB}_{\mathrm{approved}}(a)$. For example, given $G_{\widetilde{p},p'}(a,b)$, if $b\in\mathcal{LSB}_{\mathrm{approved}}(a)$, then, Alice randomly samples $G_{\widetilde{p},p'}(a,b)$ fraction of entries (excluding the fingerprinted entries) whose attribute $p$ takes value $a$ and changes them to $b$.  
% In Algorithm \ref{algo:ot_defense}, we summarize the procedure of $\mathrm{Dfs_{col}}(\mathcal{J}')$, where lines \ref{line:ot_start}-\ref{line:ot_end} solves (\ref{ot_defense}) to obtain the optimal mass transportation plan for attribute $p$, and lines \ref{line:move_start}-\ref{line:move_end} change the values of entries in $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset).p$ according to $G_{\widetilde{p},p'}$.





%\ea{Are we doing anything to maximize utility here?}

% \subsection{Advantages of $\mathrm{Dfs_{col}}(\mathcal{J}')$}
% \label{sec:adv_col_dfs}

% \hl{EA: dont have this as a subsection, it can be the last part of the previous section. You can use a bold title if you want to emphasize it. Also, I am not sure how the below paragraphs are advantages of the proposed technique.}

% As discussed in Footnote 3 \hl{EA: dont refer to foot notes, you can refer to the section}, 

% \hl{EA: can you find a more informative title for below?}
% \subsubsection{Design details of $\mathrm{Dfs_{col}}(\mathcal{J}')$.} We do not apply the optimal transportation technique to directly move the mass of the joint distributions obtained from $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$ to resemble the joint distributions in    $\mathcal{J}'$. 


% \hl{TJ: emphasize that moving the marginals can already give good defense performance? (by showing the preservation of the correlations?) what is the reason?}

% \hl{EA: you can have a different title for the below discussion}
% \subsubsection{Discussion on higher order column-wise correlation attacks.} 
% In a column-wise correlation attack, a malicious SP may also take advantage of higher-order correlations, e.g., the joint distributions of three-tuples of attributes ($J_{p,q,f}, p,q,f\in\mathcal{F}$). 
% The proposed technique is also robust against such an attack by moving the mass of $\Pr(C_{\widetilde{p}})$ to resemble 
% the marginalization of higher order joint distribution, e.g., 
% % the double marginalization of the three-tuple \hl{EA: can we say "or higher" here?} joint distribution, e.g., 
% $\Pr(C_{p'}) = \int J_{p,q,f}'dqdf$ for order 3, where $J_{p,q,f}'$ is the database owner's prior knowledge on the joint distribution of attributes $p$, $q$, and $f$. 
% % \hl{EA: ok but how does the defender know which attack the malicious SP will conduct? Can we claim marginalization of joint pairwise joint distributions are enough to mitigate such attacks?}
% Since, in practice, the database owner does not have the knowledge about which order of column-wise correlations the malicious SP will use, the proposed mitigation technique, which only considers the marginal distributions can be considered as an ``universal prescription". We experimentally validate that $\mathrm{Atk_{col}}(\mathcal{J})$ also has good performance when the malicious SP uses higher order 
% % \hl{EA: can we say "higher order" here?} 
% correlations in Appendix \ref{sec:higher_order}.






% \subsubsection{Mitigation performance analysis.} 
% % In Appendix~\ref{sec:supp_design_detail_of_dfs_col}, we elaborate more on the design details of $\mathrm{Dfs_{col}}(\mathcal{J}')$.
% % and explain why we do not  apply the optimal transportation technique to directly move the mass of the joint distributions obtained from $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$ to resemble the joint distributions in  $\mathcal{J}'$. 
% To investigate the mitigation performance of $\mathrm{Dfs_{col}}(\mathcal{J}')$ against $\mathrm{Atk_{col}}(\mathcal{J})$, one needs to study the behavior of $|J_{p,q}(a,b)-\widetilde{\widetilde{J_{p,q}}}(a,b)|$, where $\widetilde{\widetilde{J_{p,q}}}(a,b)$ denotes the new pairwise joint distributions among attributes (after mitigation). 
% However, to calculate $\widetilde{\widetilde{J_{p,q}}}(a,b)$, one requires extra knowledge about the conditional distribution among attributes of the considered database, which is not available to the database owner (to the advantage of the malicious SPs). 
% As a result, we analyze the performance of $\mathrm{Dfs_{col}}(\mathcal{J}')$ from the perspective of the Pearson’s correlations. %In particular, we can show that the database owner can arrange $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\emptyset,\mathrm{Dfs_{col}}(\mathcal{J}')\Big)$ to have  Pearson's  correlations among attribute pairs that are close to those obtained from $\overline{\mathbf{R}}\Big(\emptyset,\emptyset,\mathrm{Atk_{col}}(\mathcal{J})\Big)$ if $\mathcal{J}'$ is close to $\mathcal{J}$, which improves the robustness of the fingerprint (against correlation attacks by a malicious SP). The details are deferred to Appendix~\ref{sec:supp_design_detail_of_dfs_col}.

\subsubsection{Design details of $\mathrm{Dfs_{col}}(\mathcal{J}')$.} 
\label{sec:supp_design_detail_of_dfs_col}

We do not apply the optimal transportation technique to directly move the mass of the joint distributions obtained from $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$ to resemble the joint distributions in    $\mathcal{J}'$. 
One  reason is that, to do so, the database owner (Alice) needs to solve (\ref{ot_defense}) for  $\frac{|\mathcal{F}|(|\mathcal{F}|-1)}{2}$ joint distributions. This is computationally expensive if the  database includes a large number of attributes. Thus, by considering the mass transportation in marginal distributions, the developed mitigation technique becomes more efficient.  
Furthermore, by only considering the marginal distributions, Alice can arrange $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\emptyset,\mathrm{Dfs_{col}}(\mathcal{J}')\Big)$ to have  Pearson's  correlations among attribute pairs that are close to those obtained from $\overline{\mathbf{R}}\Big(\emptyset,\emptyset,\mathrm{Atk_{col}}(\mathcal{J})\Big)$ if $\mathcal{J}'$ is close to $\mathcal{J}$. % which helps alleviate $\mathrm{Atk_{col}}(\mathcal{J})$. 
For instance, denote the Pearson's correlation between attributes $p$ and $q$ calculated  from $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\emptyset,\mathrm{Dfs_{col}}(\mathcal{J}')\Big)$ and $\overline{\mathbf{R}}\Big(\emptyset,\emptyset,\mathrm{Atk_{col}}(\mathcal{J})\Big)$ as $\rho_{p',q'}$ and $\rho_{p,q}$, respectively. Then, we have
% \begin{equation*}
    $\rho_{p',q'} =  \frac{\sum_{a,b}(a -\mu_{C_{p'}})(b -\mu_{C_{q'}})J_{p,q}'(a,b)}{\sigma_{C_{p'}}\sigma_{C_{q'}}}$, 
% \end{equation*}
where $\mu_{C_{p'}}$ (or $\mu_{C_{q'}}$) 
and $\sigma_{C_{p'}}$ (or $\sigma_{C_{q'}}$) is the expected value   and the standard deviation  of attribute $p$ (or $q$) obtained after applying the vanilla fingerprinting scheme followed by $\mathrm{Dfs_{col}}(\mathcal{J}')$, respectively. Also, $J_{p,q}'(a,b)$ is the database owner's prior knowledge on the joint probability distribution of attribute $p$ taking value $a$ and attribute $q$ taking value $b$. Likewise, %from the malicious SP's point of view, 
% \begin{equation*}
    $\rho_{p,q} =  \frac{\sum_{a,b}(a -\mu_{C_{p}})(b -\mu_{C_{q}})J_{p,q}(a,b)}{\sigma_{C_{p}}\sigma_{C_{q}}}$, 
% \end{equation*}
where $\mu_{C_{p}}$ (or $\mu_{C_{q}}$) and 
$\sigma_{C_{p}}$ (or $\sigma_{C_{q}}$) is the expected value  and the standard deviation of attribute $p$ (or $q$) in $\overline{\mathbf{R}}\Big(\emptyset,\emptyset,\mathrm{Atk_{col}}(\mathcal{J})\Big)$. Also, $J_{p,q}(a,b)$ is the malicious SP's  prior knowledge on the joint probability distribution of attribute $p$ taking value $a$ and attribute $q$ taking value $b$. If $\mathcal{J}'$ is close to $\mathcal{J}$, then $\mu_{C_{p'}}$ (or $\mu_{C_{q'}}$) is also close to $\mu_{C_{p}}$ (or $\mu_{C_{q}}$), because of the marginalization of the similar joint distributions. Similar discussion also holds for $\sigma_{C_{p'}}$ (or $\sigma_{C_{q'}}$) and $\sigma_{C_{p}}$ (or $\sigma_{C_{q}}$). As a result, $\rho_{p',q'}$ also becomes close to $\rho_{p,q}$, which improves the robustness of the fingerprint (against correlation attacks by a malicious SP), and hence prevents a malicious SP from distorting the potentially fingerprinted positions.  



% Since the joint distributions cannot be uniquely determined from the marginal distributions, thus, 


% the new pairwise joint distributions among attributes (after mitigation)  cannot be derived from the new marginal distribution 


% are not directly obtainable. 





%  \subsubsection{Discussion on higher order column-wise correlation attacks.} 
% In a column-wise correlation attack, a malicious SP may also take advantage of higher-order correlations, e.g., the joint distributions of three-tuples of attributes ($J_{p,q,f}, p,q,f\in\mathcal{F}$). 
% The proposed technique is also robust against such an attack by just moving the mass of $\Pr(C_{\widetilde{p}})$ to resemble 
% the marginalization of  joint distribution. We will empirically corroborate this in Appendix \ref{sec:higher_order}. Since, in practice, Alice does not have the knowledge about which order of column-wise correlations the malicious SP will use, {\color{black}and she cannot explicitly model all potential correlations, the proposed mitigation technique, which only considers the marginal distributions (the most general one) can be considered as an ``universal prescription" to mitigate the impact of other column-wise correlation attacks. }




% \begin{figure}[h]
%   \begin{center}
%   \begin{tabular}{cc}
%      \includegraphics[width= .45\columnwidth]{figures/distdiff_corrdefense.eps}
% 		&
%      \includegraphics[width= .45\columnwidth]{figures/utility_corrdefense.eps}
%      \\
%     {\small  (a) Impact of CorrDefense}  &
%     {\small  (b) Utility comparison} \\
%         \end{tabular}
%       \end{center}
%   \caption{\label{fig:corrdefense} (a) Percentage of perturbed entries and the obtained $\Delta$ of $\widetilde{\mathbf{R}}$ after CorrDefense under varying $\lambda$. (b) Utility comparison between $\widetilde{\mathbf{R}}$ after CorrDefense under different $\lambda$ with $\widetilde{\mathbf{R}}$ and $\mathbf{R}$.}
% \end{figure}



\subsection{Robust Fingerprinting Against Row-wise Correlation Attack}
\label{sec:row-defense}

% \hl{EA: i didnt read this part, i think it is still incomplete}

To make a vanilla fingerprinting scheme also robust against row-wise correlation attack (in Section \ref{sec:row-wise-atack}), we develop another mitigation technique, i.e.,  $\mathrm{Dfs_{row}}(\mathcal{S}')$.
The main goal of $\mathrm{Dfs_{row}}(\mathcal{S}')$ is to avoid a malicious SP from distorting the fingerprint due to discrepancies in the expected statistical relationships between data records. 
Different from the design principle of $\mathrm{Dfs_{col}}(\mathcal{J}')$, which makes the newly obtained  joint distributions resemble the prior knowledge, we design $\mathrm{Dfs_{row}}(\mathcal{S}')$ by changing selected entries of non-fingerprinted data records to  make the newly obtained  statistical relationships as far away from Alice's prior knowledge $\mathcal{S}'$ as possible. 
This is because the row-wise correlation attack usually changes limited number of entries in the vanilla fingerprinted database (as we validate in Section \ref{sec: int_attack_census}), thus, to make the newly obtained  statistical relationships   resemble $\mathcal{S}'$, one needs to change all non-fingerprinted data records and this will significantly compromise the database utility. 
% \hl{EA: can you add something saying how this strategy (making new distributions far away from prior knowledge) makes the fingerprint robust against row-wise correlation attack?}
{\color{black}Instead, by making the new statistical relationships far away from her prior knowledge, Alice can make additional (non-fingerprinted) data records that have cumulative absolute difference (with respect to the other records in the same community) exceeding a predetermined threshold. As a result, when launching $\mathrm{Atk_{row}(\mathcal{J})}$, the malicious SP will identify wrong data records ($\boldsymbol{r}_i$), which causes $\sum_{j\neq i}^{n_c} \   \big|s_{ij}^{\mathrm{comm}_c}-\widetilde{s_{ij}}^{\mathrm{comm}_c}\big| \geq \tau_{\mathrm{row}}^{\mathrm{Atk}}$, and hence change the non-fingerprinted records.}

In $\mathrm{Dfs_{row}}(\mathcal{S}')$, Alice selects a subset of  non-fingerprinted data records in a community $c$, i.e., $\mathcal{E}_c\subset\mathrm{comm}_c, c\in[1,C]$, and changes their value to   $\widetilde{\widetilde{\boldsymbol{r}_i}}, i\in\mathcal{E}_c$, such that the cumulative absolute  difference  between statistical relationships in her prior knowledge and those obtained from the   fingerprinted database  achieves the maximum difference   after   applying   $\mathrm{Dfs_{row}}(\mathcal{S}')$. This can be formulated  as  the following optimization problem:
% \begin{equation}
% \begin{aligned}
% \max_{\mathcal{E}_c} \quad &  d(\mathcal{E}_c)=    \sum_{j\in  \mathrm{comm}_c/\mathcal{E}_c}\sum_{i\in\mathcal{E}_c} \   \Big|{s'_{ij}}^{\mathrm{comm}_c}-\widetilde{\widetilde{s_{ij}}}^{\mathrm{comm}_c}\Big| \\
% \textrm{s.t.} \quad & \mathcal{E}_c\subset \mathrm{comm}_c/\mathcal{Q}_c,\\
%   & \widetilde{\widetilde{s_{ij}}}^{\mathrm{comm}_c} = e^{-\mathrm{dist}(\widetilde{\widetilde{\boldsymbol{r}_i}},\boldsymbol{r}_j)}, i\in\mathcal{E}_c,j \in\mathrm{comm}_c/\mathcal{E}_c\\
%     &  |\mathcal{E}_c|\leq \left \lceil{n_c\gamma}\right \rceil,   
% \end{aligned}
% \label{eq:row_defense}
% \end{equation}




\begin{equation}
\begin{aligned}
\max_{\mathcal{E}_c,\widetilde{\widetilde{\boldsymbol{r}_i}}} \quad &  d(\mathcal{E}_c)=   \Big| \sum_{j\in  \mathrm{comm}_c/\mathcal{E}_c}\sum_{i\in\mathcal{E}_c} \   \Big|{s'_{ij}}^{\mathrm{comm}_c}-\widetilde{\widetilde{s_{ij}}}^{\mathrm{comm}_c}\Big| \\
& \qquad\quad -\sum_{j\in  \mathrm{comm}_c/\mathcal{E}_c}\sum_{i\in\mathcal{E}_c} \   \Big|{s'_{ij}}^{\mathrm{comm}_c}- \widetilde{s_{ij}}^{\mathrm{comm}_c}\Big| \Big| \\
\textrm{s.t.} \quad & \mathcal{E}_c\subset \mathrm{comm}_c/\mathcal{Q}_c,\\
   & \widetilde{\widetilde{s_{ij}}}^{\mathrm{comm}_c} = e^{-\mathrm{dist}(\widetilde{\widetilde{\boldsymbol{r}_i}},\boldsymbol{r}_j)}, i\in\mathcal{E}_c,j \in\mathrm{comm}_c/\mathcal{E}_c,\\
   & \widetilde{\widetilde{\boldsymbol{r}_i}} = \mathrm{value\  change}(\widetilde{\boldsymbol{r}_i}), i \in\mathcal{E}_c,\\
    &  |\mathcal{E}_c|\leq \left \lceil{n_c\gamma}\right \rceil,
\end{aligned}
\label{eq:row_defense}
\end{equation}
$\forall c\in[1,C]$. $\mathcal{Q}_c$ is the set of fingerprinted records in community $c$, ${s_{ij}'}^{\mathrm{comm}_c}$ denotes Alice's prior knowledge on  the statistical relationship between individuals $i$ and $j$ in community $c$,  $\widetilde{s_{ij}}^{\mathrm{comm}_c}$ is the   statistical relationship between individuals $i$ and $j$ in community $c$ in $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$, whose $i$th data record is denoted as $\widetilde{\boldsymbol{r}_i}$, 
and  $\widetilde{\widetilde{s_{ij}}}^{\mathrm{comm}_c}$ is such information  obtained from  $\widetilde{\mathbf{R}}(\mathrm{FP},\mathrm{Dfs_{row}}(\mathcal{S}'),\emptyset)$, whose $i$th data record is represented as $\widetilde{\widetilde{\boldsymbol{r}_i}}$. Also, $\mathrm{value\ change}(\cdot)$ is the function that changes each attribute of $\widetilde{\boldsymbol{r}_i}$, and it will be elaborated later. In (\ref{eq:row_defense}), we let the  cardinality of $\mathcal{E}_c$ to  be smaller than $\left \lceil{n_c\gamma}\right \rceil$ ($\gamma$ is the percentage of fingerprinted records)  to   restrict the number of selected non-fingerprinted records to maintain database utility.

% Solution to 
(\ref{eq:row_defense}) is an NP-hard  combinatorial search problem \cite{bertsimas1997introduction}. 
% as it can be reduced from the knapsack problem 
Thus,  we use a greedy algorithm to determine $\mathcal{E}_c$ and a heuristic approach to obtain $\widetilde{\widetilde{\boldsymbol{r}_i}}, i\in\mathcal{E}_c$.   In fact, (\ref{eq:row_defense}) also belongs to the problems of set function maximization, which can be connected  to submodular optimization \cite{wei2015submodularity}, and     greedy algorithms are widely used for   selecting candidate sets. Specifically, Alice   constructs     $\mathcal{E}_c$ by greedily      choosing up to  $\left \lceil{n_c\gamma}\right \rceil$   non-fingerprinted  data records (in $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$) that  have the maximum cumulative absolute difference (i.e., $\sum_{j\in  \mathrm{comm}_c,j\neq i}^{n_c} \\  \big|{s'_{ij}}^{\mathrm{comm}_c}-  \widetilde{s_{ij}}^{\mathrm{comm}_c}\big|,i\in\mathrm{comm}_c/\mathcal{Q}_c$) with Alice's prior knowledge ($\mathcal{S}'$). %, i.e., $\sum_{j\in  \mathrm{comm}_c/\mathcal{E}_c}\sum_{i\in\mathcal{E}_c}  \big|{s'_{ij}}^{\mathrm{comm}_c}- \\  \widetilde{s_{ij}}^{\mathrm{comm}_c}\big|$ is minimized.
Next, she changes   the value of each attribute  of the selected data records in  $\mathcal{E}_c$ to the most frequent occurring instance of that attribute to obtain $\widetilde{\widetilde{\boldsymbol{r}_i}}$ (i.e.,  $\widetilde{\widetilde{\boldsymbol{r}_i}} = \mathrm{value\  change}(\widetilde{\boldsymbol{r}_i})$).
% so as to increase the value of $\sum_{j\in  \mathrm{comm}_c/\mathcal{E}_c}\sum_{i\in\mathcal{E}_c}     \big|{s'_{ij}}^{\mathrm{comm}_c}-\widetilde{\widetilde{s_{ij}}}^{\mathrm{comm}_c}\big|$. 
We   describe the steps to apply $\mathrm{Dfs_{row}}(\mathcal{S}')$ in Algorithm \ref{algo:row-wise-defense}. % in Appendix~\ref{sec:supp_algos_row_wise_defense}. 


\begin{algorithm}
\small
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Vanilla fingerprinted database, $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$, fingerprinting ratio $\gamma$, database owner's prior knowledge on the row-wise correlations  $\mathcal{S}'$ and individuals' affiliation to the $C$ communities.}
\Output{$\widetilde{\mathbf{R}}\Big(\mathrm{FP},\mathrm{Dfs_{row}}(\mathcal{S}'),\emptyset,\Big)$.}

Obtain $\widetilde{\mathcal{S}}$, i.e.,  the   set of  pairwise statistical relationships among individuals in each community,   from the vanilla fingerprinted database $\widetilde{\mathbf{R}}(\mathrm{FP},\emptyset,\emptyset)$;

\ForAll{$\mathrm{comm}_c, c\in[1,C]$}{\ForAll{non-fingerprinted individual $i\in \mathrm{comm}_c/\mathcal{Q}_c$}{

Calculate %the cumulative statistical relationships of individual $i$ with the rest of the records in  $\mathrm{comm}_c$ as 
$e_i = \sum_{j\in  \mathrm{comm}_c,j\neq i}^{n_c}  \big|{s'_{ij}}^{\mathrm{comm}_c}-  \widetilde{s_{ij}}^{\mathrm{comm}_c}\big|, i\in\mathrm{comm}_c/\mathcal{Q}_c$;

}

Obtain the largest $\left \lceil{n_c\gamma}\right \rceil$ $e_i$'s, and collect these row index $i$ in set $\mathcal{E}_c$;


\ForAll{row index $i\in\mathcal{E}_c$}{

$\widetilde{\widetilde{\boldsymbol{r}_i}} = \mathrm{value\  change}(\widetilde{\boldsymbol{r}_i})$;
\CommentSty{//change the value of each attribute of $\widetilde{\boldsymbol{r}_i}$ to the most frequently  occurred instance of that attribute in $\mathrm{comm}_c$.\\}
}

}


 
 Return $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\mathrm{Dfs_{row}}(\mathcal{S}'),\emptyset,\Big)$.

		\caption{$\mathrm{Dfs_{row}}(\mathcal{S}')$: defense against row-wise correlation attack.}
\label{algo:row-wise-defense}
\end{algorithm}

The   solution to (\ref{eq:row_defense}) depends on the database and the distribution of data entries, thus, it is infeasible to derive a generic closed-form expression to  quantify the mitigation performance of $\mathrm{Dfs_{row}}(\mathcal{S}')$. However, in Section \ref{sec:exp_defense_on_census}, we will empirically show that the fraction of the fingerprinted entries inferred by $\mathrm{Atk_{row}}(\mathcal{S})$ will decrease significantly if Alice applies the post-processing step $\mathrm{Dfs_{row}}(\mathcal{S}')$. 


% {\color{blue}In the future work, we will }






% \hl{EA: this may need a subtitle/subsection like "integrated robust fingerprinting algorithm"}
\subsection{Integrated Robust Fingerprinting}
Although after applying  $\mathrm{Dfs_{row}}(\mathcal{S}')$, the malicious SP may still identify (and distort) some fingerprinted data records using $\mathrm{Atk_{row}}(\mathcal{J})$, the amount of distortion in the fingerprint will not be enough to compromise the fingerprint bit-string due to the majority voting considered in the vanilla scheme. In Section \ref{sec: int_attack_census}, we validate that Algorithm \ref{algo:row-wise-defense} can successfully mitigate the row-wise correlation attack in a real-world  database. Since $\mathrm{Dfs_{row}}(\mathcal{S}')$ changes less number of entries than $\mathrm{Dfs_{col}}(\mathcal{J}')$, database owner will apply $\mathrm{Dfs_{row}}(\mathcal{S}')$ first after the vanilla fingerprinting.  In Algorithm \ref{algo:robust-fp}, we summarize the main steps of our integrated robust fingerprinting scheme against the identified correlation attacks.

\begin{algorithm}
\small
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{A database $\mathbf{R}$, a vanilla fingerprinting scheme $\mathrm{FP}$, database owner's prior knowledge on the column-wise and row-wise correlation, i.e., $\mathcal{J}'$ and $\mathcal{S}'$, and individuals' affiliation to the $C$ communities.}

\Output{$\widetilde{\mathbf{R}}\Big(\mathrm{FP},\mathrm{Dfs_{row}}(\mathcal{S}'),\mathrm{Dfs_{col}}(\mathcal{J}')\Big)$.}

 

Apply the vanilla fingerprinting scheme on $\mathbf{R}$ and obtain $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\emptyset,\emptyset\Big)$;

Apply  $\mathrm{Dfs_{row}}(\mathcal{S}')$  on  $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\emptyset,\emptyset\Big)$ using Algorithm \ref{algo:row-wise-defense} and obtain $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\mathrm{Dfs_{row}}(\mathcal{S}'),\emptyset\Big)$;

Apply  $\mathrm{Dfs_{col}}(\mathcal{J}')$ on $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\mathrm{Dfs_{row}}(\mathcal{S}'),\emptyset\Big)$ using Algorithm \ref{algo:ot_defense} and obtain $\widetilde{\mathbf{R}}\Big(\mathrm{FP},\mathrm{Dfs_{row}}(\mathcal{S}'),\mathrm{Dfs_{col}}(\mathcal{J}')\Big)$;

		\caption{Robust fingerprinting against correlation attacks.}
\label{algo:robust-fp}
\end{algorithm}




% $\sum_{j\neq i}^{n_c} \   \big|s_{ij}^{\mathrm{comm}_c}-\widetilde{s_{ij}}^{\mathrm{comm}_c}\big| \geq \tau$

% \hl{We need to have a single proposed fingerprinting scheme combining both considered defenses (if possible lets also consider a general figure summarizing the whole process). Also, we should discuss/show the robustness and utility guarantees of the proposed fingerprinting scheme (by using a similar analysis as in BS or Tardos codes).}

% \hlgreen{TJ: for the ``single proposed fingerprinting scheme combining both considered defenses'', do we just give s very short algorithm with only three steps: 1. vanilla FP, 2. row wise mitigation, 3 column-wise mitigation?} \hl{EA: yes, after you describe the individual (row and column wise) defenses in detail, you can then discuss how they will be used together briefly}






% \subsection{Prior Knowledge Asymmetry at Column-wise Augmented Flipping Attack and Defense}


% \subsection{Prior Knowledge Asymmetry at Row-wise Augmented Flipping Attack and Defense}


% %To handle the scenario where the row-wise correlation models used by the malicious SPs are different with that 




% We denote the ground truth individuals' relationship knowledge    as $\mathbf{A}$, individuals' relationship knowledge obtained from the fingerprinted database as $\widetilde{\mathbf{A}}$, and the individuals' relationship knowledge used by the database owner (resp. service provider) as $\mathbf{A}^{\mathrm{owner}}$ (resp. $\mathbf{A}^{\mathrm{SP}}$). 



% To model the discrepancy between $\mathbf{A}$ and $\mathbf{A}^{\mathrm{owner}}$, and between $\mathbf{A}$ and $\mathbf{A}^{\mathrm{SP}}$, we consider 

% \begin{equation*}
%     \begin{aligned}
%      a^{\mathrm{owner}}_{ij} &= a_{ij} + N^{\mathrm{owner}}_{ij},\qquad & i,j\in[1,N],i\neq j,\\
%       a^{\mathrm{SP}}_{ij} &= a_{ij} + N^{\mathrm{SP}}_{ij},\qquad & i,j\in[1,N],i\neq j,
%     \end{aligned}
% \end{equation*}
%  where $N^{\mathrm{owner}}_{ij}$ (resp. $N^{\mathrm{SP}}_{ij}$) is a Gaussian distributed noise that affects database owner's (resp. service provider's) apriori knowledge.  In particular, we assume both noises are Gaussian distributed with zero mean but different variance, i.e., 
%  $N^{\mathrm{owner}}_{ij}\sim \mathcal{N}(0,\sigma_{\mathrm{owner}}^2)$
%  and  $N^{\mathrm{SP}}_{ij}\sim \mathcal{N}(0,\sigma_{\mathrm{SP}}^2)$. Besides, both $\sigma_{\mathrm{owner}}^2$ and $\sigma_{\mathrm{SP}}^2$ are unknown to the database owner and the malicious  SP.
 
 
%  Then, the probability of an attacker   regards individual   $i$'s record  as a fingerprinted record is
% \begin{equation*}
% \begin{aligned}
%   p_i&= \Pr\Bigg(    \sum_{j\neq i}^N \   \Big(a^{\mathrm{SP}}_{ij}-\widetilde{a}_{ij}\Big)^2 \geq \Delta \Bigg) =     \Pr\Bigg(    \sum_{j\neq i}^N \   \Big(a_{ij} + N^{\mathrm{SP}}_{ij}-\widetilde{a}_{ij}\Big)^2 \geq \Delta \Bigg)\\
%   & \stackrel{*} = \Pr\Bigg(    \sum_{j\neq i}^N \   \Big(a_{ij} + N^{\mathrm{SP}}_{ij}-a_{ij}-\delta\Big)^2 \geq \Delta \Bigg)
%   \end{aligned}
% \end{equation*}

% \begin{prop} The expected number of individual recorded being attacked by the row-wise augmented correlation attack under asymmetric row-wise correlation model satisfies $ \mathbb{E}[T]  \in \Big[\sum_{i=1}^N l_i  , \sum_{i=1}^N u_i\Big]$, where $l_i =  \frac{1}{\Gamma((N-1)/2)}\gamma \Bigg(\frac{N-1}{2}, \frac{\Delta + \sum_{j\neq i}^N (a_{ij} -\widetilde{a}_{ij})^2}{2}\Bigg)$ and\\ $u_i = 1- \frac{1}{\Gamma((N-1)/2)}\gamma \Bigg(\frac{N-1}{2}, \frac{\Delta - \sum_{j\neq i}^N (a_{ij} -\widetilde{a}_{ij})^2}{2}\Bigg)$.\footnote{$\Gamma(s)$ is the Gamma function, i.e, $\Gamma(s) = \int_0^{\infty} t^{s-1}e^{-t}dt$, and $\gamma(s,x)$ is the lower incomplete gamma function i.e., $\gamma(s,x) = \int_0^x t^{s-1} e^{-t} dt$.} 
% \label{prop:p_row}
% \end{prop}
% \begin{proof}  




% %Define random variable $X_{ij}  = a_{ij} + N_{ij}-\widetilde{a}_{ij}$. Since $N_{ij}\sim \mathcal{N}(0,\sigma^2)$ and $X_{ij} \sim \mathcal{N}(a_{ij}-a'_{ij},\sigma^2)$, and

% Since $\{N_{ij} | \sum_{j\neq i}^N \   (a_{ij} + N_{ij}-\widetilde{a}_{ij})^2 \geq \Delta\} \subset \{N_{ij} | \sum_{j\neq i}^N \  N_{ij}^2 + (a_{ij} -\widetilde{a}_{ij})^2 \geq \Delta\} $. We can have  
% \begin{equation*}
% \begin{aligned}
% p_i&\leq \Pr\Big(\sum_{j\neq i}^N \  N_{ij}^2 \geq \Delta - \sum_{j\neq i}^N (a_{ij} -\widetilde{a}_{ij})^2 \Big) \\
% &\stackrel{*}= 1- \frac{1}{\Gamma((N-1)/2)}\gamma \Bigg(\frac{N-1}{2}, \frac{\Delta - \sum_{j\neq i}^N (a_{ij} -\widetilde{a}_{ij})^2}{2}\Bigg) = u_i,
% \end{aligned}
% \end{equation*}
% where $(*)$ is because $\sum_{j\neq i}^N \  N_{ij}^2 \sim \mathcal{X}^2_{N-1}$, i.e., chi-square distribution with $N-1$ degrees of freedom.

% Likewise, since $\{N_{ij} | \sum_{j\neq i}^N \   (a_{ij} + N_{ij}-\widetilde{a}_{ij})^2 \geq \Delta\} \supset \{N_{ij} | \sum_{j\neq i}^N \  N_{ij}^2 - (a_{ij} -\widetilde{a}_{ij})^2 \geq \Delta\} $. We can have  
% \begin{equation*}
% \begin{aligned}
% p_i&\geq \Pr\Big(\sum_{j\neq i}^N \  N_{ij}^2 \geq \Delta + \sum_{j\neq i}^N (a_{ij} -\widetilde{a}_{ij})^2 \Big) \\
% &=  \frac{1}{\Gamma((N-1)/2)}\gamma \Bigg(\frac{N-1}{2}, \frac{\Delta + \sum_{j\neq i}^N (a_{ij} -\widetilde{a}_{ij})^2}{2}\Bigg) = l_i.
% \end{aligned}
% \end{equation*}

% Since the attacker will launch the row-wise correlation flipping attack on record $i$ if $\mathbf{1}\Big\{    \sum_{j\neq i}^N \   (a'_{ij}-\widetilde{a}_{ij})^2 \geq \Delta \Big\} = 1$, where $\mathbf{1}\{\cdot\}$ is the indicator function. As a result, the number of attacked individual records (T) is a collection of $N$ independent yes or no trials with success probabilities determined by $p_i, i\in[1,N]$. According to \cite{}, $T$ is Poisson binomial distributed random variable with mean $\sum_{i=1}^N p_i$, which gives $\sum_{i=1}^N l_i \leq \mathbb{E}[T] \leq \sum_{i=1}^N u_i$.
% \end{proof}

==> sections/related_work.tex <==
\section{Related Work}
\label{sec:related_work}



% Here, 

We first briefly review the works on multimedia fingerprinting, and then focus on existing works on fingerprinting relational database. 


Large volume of research on  watermarking and fingerprinting  have targeted multimedia, e.g.,  images~\cite{van1994digital,gonge2013robust}, audio \cite{bassia2001robust,  kirovski2001robust},  videos~\cite{swanson1998multiresolution}, and text documents~\cite{Brassil94hidinginformation,Brassil1995}. Such works benefit from the high redundancy in
multimedia, such that the inserted watermark or fingerprint is imperceptible for human beings.    However, the aforementioned multimedia fingerprinting techniques cannot be applied to fingerprint relational databases. The reason is that a database fingerprinting scheme should be robust against common database operations, such as union, intersection, and updating, whereas multimedia fingerprinting schemes are designed to be robust against operations, like compression and formatting.


Database fingerprinting schemes are usually discussed together with database watermarking schemes \cite{li2003constructing} due to their similarity. 
In the seminal work \cite{agrawal2003watermarking}, Agrawal et al. introduce a watermarking framework for relations with numeric attributes by assuming that the database consumer can tolerate a small amount of error in the watermarked databases. Then, based on \cite{agrawal2003watermarking}, some database fingerprinting schemes have been devised. Specifically, Guo et al. \cite{guo2006fingerprinting} develop a two-stage fingerprinting scheme: the first stage is used to prove database ownership, and the second stage is designed for extracted fingerprint verification. Li et al.~\cite{li2005fingerprinting} develop a database fingerprinting scheme by extending \cite{agrawal2003watermarking} to enable the insertion and extraction of arbitrary bit-strings in relations. Furthermore, the authors provide an extensive robustness analysis (e.g., about the upper bound on the probability of detecting incorrect but valid fingerprint from the pirated database) of their scheme. Although \cite{guo2006fingerprinting,li2005fingerprinting} pseudorandomly determine the fingerprint positions in a database, they are not robust against our identified correlation attacks. 
In this paper, we consider \cite{li2005fingerprinting}  as the vanilla fingerprinting scheme and corroborate its vulnerability against correlation attacks. 
Additionally, Liu et al. \cite{liu2004block} propose a  database fingerprinting scheme by dividing  the relational database into blocks and ensuring that certain bit positions of the data at certain blocks contain specific values. In~\cite{liu2004block},  since the fingerprint is embedded block-wise, it is more susceptible to attacks utilizing correlations in the data. 
As a result, incorporating data correlations in database fingerprint schemes is critical to provide robustness against correlation attacks.   

 
Recently,  Yilmaz et al. \cite{yilmaz2020collusion} develop a probabilistic fingerprinting scheme by explicitly considering the correlations (in terms of conditional probabilities) between data points in data record of a single individual. Ayday et al.~\cite{ayday2019robust} propose an optimization-based fingerprinting scheme for sharing  personal sequential data by minimizing the probability of collusion attack with data correlation being one of the constraints. Our work differs from these works since we focus on  developing robust fingerprint scheme for relational databases, which (i) contain large amount of data records from different individuals, (ii) include both column- and row-wise correlations, and (iii) have different utility requirements.  



